AIM: Automated Input Set Minimization for Metamorphic Security Testing

Although the security testing of Web systems can be automated by generating crafted inputs, solutions to automate the test oracle, i.e., vulnerability detection, remain difficult to apply in practice. Specifically, though previous work has demonstrated the potential of metamorphic testing, security failures can be determined by metamorphic relations that turn valid inputs into malicious inputs, metamorphic relations are typically executed on a large set of inputs, which is time-consuming and thus makes metamorphic testing impractical. We propose AIM, an approach that automatically selects inputs to reduce testing costs while preserving vulnerability detection capabilities. AIM includes a clustering-based black-box approach, to identify similar inputs based on their security properties. It also relies on a novel genetic algorithm to efficiently select diverse inputs while minimizing their total cost. Further, it contains a problem-reduction component to reduce the search space and speed up the minimization process. We evaluated the effectiveness of AIM on two well-known Web systems, Jenkins and Joomla, with documented vulnerabilities. We compared AIM's results with four baselines involving standard search approaches. Overall, AIM reduced metamorphic testing time by 84% for Jenkins and 82% for Joomla, while preserving the same level of vulnerability detection. Furthermore, AIM significantly outperformed all the considered baselines regarding vulnerability coverage.

==> Appendices/proofs_problemDef.tex <==
\section{Formal results for the Problem Definition}
%\label{sec:aim:appendix:framework}


%%%%%%%%%%%%%%%%
\subsection{Input Coverage and Cost}
\label{sec:aim:appendix:assumptions}

\begin{lem}[Non-Empty Coverage]
\label{theo:SubclassesNotEmpty}
    For every input $\sequence$, we have $\getSubclasses{\sequence} \neq \varnothing$.
\end{lem}

\begin{proof}
    We consider only inputs containing at least one action (\S VI-B). %(\Cref{defi:sequences}).
    Let $\action_1 = \getAction{\sequence}{1}$ be the first action of $\sequence$.
    $\action_1$ has an output in $\outputClass_1 = \getOutputClass{\sequence}{1}$ (\S VI-B).% (\Cref{defi:outputClassOfAction}).
    $\action_1$ is in the action set $\actionClass_1 = \getActionClass{\outputClass_1}$ (\S VI-C). %(\Cref{defi:actionClass}).
    After clustering of this action set, let
    $\actionSublass_1 = \getSubclassFromAct{\sequence}{1} = \getActionSubclass{\action_1}{\actionClass_1}$
    be the input block of the action $\action_1$ executed in $\sequence$ (\S VI-C). % (\Cref{defi:actionSubclassesFromSequence}).
    Therefore, we have $\actionSublass_1 \in \getSubclasses{\sequence}$.
\end{proof}

\begin{lem}[Cost is Positive]
\label{theo:costPositive}
    For every input $\sequence$, we have $\costFunction{\sequence} > 0$.
    For every input set $\TestSuite$, we have $\costFunction{\TestSuite} \ge 0$, and $\costFunction{\TestSuite} = 0$ if and only if $\TestSuite = \varnothing$.
\end{lem}

\begin{proof}
    Since we removed inputs with no cost (\S III-A), % (\Cref{sec:aim:cost}),
    for each input $\sequence$, $\costFunction{\sequence} > 0$.
    The cost of an input set is the sum of the cost of its inputs, hence $\costFunction{\TestSuite} \ge 0$.
    In particular, if $\TestSuite = \varnothing$, then $\costFunction{\TestSuite} = 0$.
    Finally, because the cost is positive, the only case where $\costFunction{\TestSuite} = 0$ is when $\TestSuite = \varnothing$.
\end{proof}


%%%%%%%%%%%%%%%%
\subsection{Redundancy}
\label{sec:aim:appendix:redundancy}

In this section, we prove that our characterization of redundancy is sound regarding the coverage of an input set (\Cref{theo:redundantSound}), then we introduce \Cref{theo:removingSeq} which is useful to prove \Cref{theo:redundantReduction} in \Cref{sec:aim:appendix:validOrders}
and \Cref{theo:redundantComps} in \Cref{sec:aim:appendix:subproblem}.

First, if an input $\sequence$ is in the considered input set $\TestSuite$, then its redundancy is not negative.
Indeed, there is always at least one input in $\TestSuite$ that covers the input blocks covered by $\sequence$, which is $\sequence$ itself.

\begin{lem}[Redundancy is Non-negative]
\label{theo:redundancy}
    Let $\TestSuite$ be an input set and $\sequence$ be an input.
    If $\sequence \in \TestSuite$, then $\redundancy{\sequence}{\TestSuite} \ge 0$.
\end{lem}

\begin{proof}
Let $\sequence$ be an input in $\TestSuite$.
Let $\actionSublass \in \getSubclasses{\sequence}$ be any block covered by $\sequence$.
Because $\actionSublass \in \getSubclasses{\sequence}$, we have that $\sequence \in \getSequences{\actionSublass}$ (\S III-A). %(\Cref{defi:coveringSeqs}).
Moreover, $\sequence \in \TestSuite$, so $\sequence \in \getSequences{\actionSublass} \cap \TestSuite$, thus we have $\superposition{\actionSublass}{\TestSuite} \ge 1$ (\S III-C). %(\Cref{defi:superposition}).
Therefore, for any $\actionSublass \in \getSubclasses{\sequence}$ we have $\superposition{\actionSublass}{\TestSuite} \ge 1$.
So, $\min \set{\superposition{\actionSublass}{\TestSuite}}{\actionSublass \in \getSubclasses{\sequence}} \ge 1$. By subtracting 1, we have $\redundancy{\sequence}{\TestSuite} \ge 0$ (\S III-C). % (\Cref{defi:redundancy}).
\end{proof}

We prove that our characterization of redundancy is sound regarding the coverage of an input set.
In other words, if an input is redundant in an input set, then it can be removed without reducing the coverage of the input set:

\begin{prop}[Redundancy Soundness]
\label{theo:redundantSound}
\label{theo:appendix:redundantSound}
    Let $\TestSuite \subseteq \TestSuiteInit$ be an input set and $\sequence \in \TestSuite$.
    If $\sequence \in \Redundant{\TestSuite}$, then $\getSubclasses{\TestSuite \setminus \set{\sequence}{}} = \getSubclasses{\TestSuite}$.
\end{prop}

\begin{proof}
%If $\sequence \not\in \TestSuite$ then $\TestSuite \setminus \set{\sequence}{} = \TestSuite$, thus $\getSubclasses{\TestSuite \setminus \set{\sequence}{}} = \getSubclasses{\TestSuite}$.
%
%Otherwise, $\sequence \in \TestSuite$.
%In that case,
$\getSubclasses{\TestSuite} = \getSubclasses{\TestSuite \setminus \set{\sequence}{}} \cup \getSubclasses{\sequence}$ (\S VI-C). % (\Cref{defi:actionSubclassesFromSequence}).
We assume that $\sequence$ is redundant in $\TestSuite$.
So, according to \Cref{theo:redundancy}, we have $\redundancy{\sequence}{\TestSuite} > 0$ (\S III-C). % (\Cref{defi:redundantSeq}).
Thus, for each $\actionSublass \in \getSubclasses{\sequence}$, we have that $\superposition{\actionSublass}{\TestSuite} \ge 2$.
Hence, according to our definition of superposition (\S III-C), % (\Cref{defi:superposition}),
there are at least two inputs $\sequence_1$ and $\sequence_2$ in $\TestSuite$ which also belong to $\getSequences{\actionSublass}$.
Because we have $\actionSublass \in \getSubclasses{\sequence}$, we have that $\sequence \in \getSequences{\actionSublass}$ (\S III-A). % (\Cref{defi:coveringSeqs}).
So, $\sequence$ is one of these inputs.
We assume this is the first one i.e., $\sequence_1 = \sequence$.
Therefore, for each $\actionSublass \in \getSubclasses{\sequence}$, there exists an input $\sequence_2 \in \getSequences{\actionSublass} \cap \TestSuite$ which is not $\sequence$.
We denote $\sequence_2 = \sequence_{\actionSublass}$ this input.
For each $\actionSublass \in \getSubclasses{\sequence}$, we have $\sequence_{\actionSublass} \in \getSequences{\actionSublass}$.
So, we have $\actionSublass \in \getSubclasses{\sequence_{\actionSublass}}$ (\S III-A). % (\Cref{defi:coveringSeqs}).
Moreover, $\sequence_{\actionSublass} \in \TestSuite$ and is not $\sequence$, so is in $\TestSuite \setminus \set{\sequence}{}$.
Thus (\S VI-C) % (\Cref{defi:actionSubclassesFromSequence})
we have $\actionSublass \in \getSubclasses{\TestSuite \setminus \set{\sequence}{}}$.
Therefore, $\getSubclasses{\sequence} \subseteq \getSubclasses{\TestSuite \setminus \set{\sequence}{}}$.
Finally, $\getSubclasses{\TestSuite} = \getSubclasses{\TestSuite \setminus \set{\sequence}{}} \cup \getSubclasses{\sequence} = \getSubclasses{\TestSuite \setminus \set{\sequence}{}}$.
\end{proof}

Finally, removing an input in an input set may update the redundancy of other inputs:

\begin{lem}[Removing an Input]
\label{theo:removingSeq}
    Let $\TestSuite$ be an input set and $\sequence_2, \sequence_1 \in \TestSuite$ be two inputs in this input set.
    $$
    \begin{array}{r@{}l}
         \redundancy{\sequence_1}{\TestSuite} - 1 &{} \le \redundancy{\sequence_1}{\TestSuite \setminus \set{\sequence_2}{}}  \\
         &{} \le \redundancy{\sequence_1}{\TestSuite}
    \end{array}
    $$
\end{lem}

\begin{proof}
    Let $\actionSublass \in \getSubclasses{\sequence_1}$.
    We denote $c_1 = \card{\getSequences{\actionSublass} \cap \TestSuite}$ and $c_2 = \card{\getSequences{\actionSublass} \cap (\TestSuite \setminus \set{\sequence_2}{})}$.
    If $\sequence_2 \in \getSequences{\actionSublass}$ then $c_2 = c_1 - 1$.
    Otherwise, $c_2 = c_1$.
    Therefore, for every $\actionSublass \in \getSubclasses{\sequence_1}$ we have $c_1 - 1 \le c_2 \le c_1$.
    This includes the input blocks minimizing the cardinality in the definition of redundancy (\S III-C). % (\Cref{defi:redundancy}).
    Hence the result.
\end{proof}


%%%%%%%%%%%%%%%%
\subsection{Valid Orders of Removal Steps}
\label{sec:aim:appendix:validOrders}

In this section, we first prove \Cref{theo:orderWithoutRepetition} that establishes that orders of removal steps contain inputs without repetition.
Then, we introduce \TSE{2.6}{subsequences} and prove \Cref{theo:sublists}, used in the rest of the section and in proofs of \Cref{sec:aim:appendix:subproblem}.
Finally, we prove \Cref{theo:canonicalOrder} presented in \S III-C. %  \Cref{sec:aim:gain}.

\begin{lem}[Order without Repetition]
\label{theo:orderWithoutRepetition}
    Let $\TestSuite$ be an input set.
    If $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, then $\sequence_1, \dots, \sequence_n$ are distinct.
\end{lem}

\begin{proof}
The proof is done by induction on $n$.

If $n = 0$, then $\dataList{\sequence_1, \dots, \sequence_n} = \dataList{}$ is empty, hence there are no two identical inputs.

We now consider $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\TestSuite}$.
By induction hypothesis, $\sequence_1, \dots, \sequence_n$ are distinct.
According to the definition of valid order of removal steps (\S III-C), % (\Cref{defi:validSteps}),
we have $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}}$ only if $\sequence_{n + 1} \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}$.

Since $\Redundant{\TestSuite} = \set{\sequence \in \TestSuite}{\redundancy{\sequence}{\TestSuite} > 0}$, we have $\sequence_{n + 1} \in \TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}$.

Therefore, $\sequence_{n + 1}$ is distinct from the previous inputs $\sequence_1, \dots, \sequence_n$.
Hence the result, which concludes the induction step.
\end{proof}

\begin{lem}[Redundant Inputs After Reduction]
\label{theo:redundantReduction}
    Let $\TestSuite$ be an input set.
    For each subset of inputs $\set{\sequence_1, \dots, \sequence_n}{} \subseteq \TestSuite$, we have $\Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} \subseteq \Redundant{\TestSuite}$.
\end{lem}

\begin{proof}
The proof is done by induction on $n$.

If $n = 0$ then $\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{} = \TestSuite$, hence the result.

Otherwise, we assume by induction that $\Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} \subseteq \Redundant{\TestSuite}$.

According to \Cref{theo:removingSeq}, redundancies can only decrease when performing a removal step.
So, for every input $\sequence_0 \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}}{}}$, we have:
$$
\begin{array}{r@{}l}
     0 &{} < \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}}{}}  \\
     &{} \le \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} 
\end{array}
$$

So, $\Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}}{}} \subseteq \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} \subseteq \Redundant{\TestSuite}$.
\end{proof}

Since orders of removal steps contain inputs without repetition (\Cref{theo:orderWithoutRepetition}), the index $\listIndex{\sequence}{\ell}$ of an input $\sequence$ in a removal order $\ell$ containing $\sequence$ is well defined.
We leverage this to define \TSE{2.6}{subsequences}.

\begin{defi}[Subsequences]
\label{defi:sublists}
Let $\dataList{\sequence_1, \dots, \sequence_n}$ and $\dataList{\sequence'_1, \dots, \sequence'_m}$ be two orders of removal steps.
We say that $\dataList{\sequence'_1, \dots, \sequence'_m}$ is a \emph{\TSE{2.6}{subsequence}} of $\dataList{\sequence_1, \dots, \sequence_n}$ \TSE{2.6}{if $\dataList{\sequence'_1, \dots, \sequence'_m}$ can be obtained by removing some elements of $\dataList{\sequence_1, \dots, \sequence_n}$, i.e.,} if 
$\set{\sequence \in \dataList{\sequence'_1, \dots, \sequence'_m}}{} \subseteq \set{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}}{}$
and,
%the ordering is preserved i.e.,
for any two inputs $\sequence_i, \sequence_j \in \dataList{\sequence'_1, \dots, \sequence'_m}$, if
$\listIndex{\sequence_i}{\dataList{\sequence_1, \dots, \sequence_n}} \le \listIndex{\sequence_j}{\dataList{\sequence_1, \dots, \sequence_n}}$,
then $\listIndex{\sequence_i}{\dataList{\sequence'_1, \dots, \sequence'_m}} \le \listIndex{\sequence_j}{\dataList{\sequence'_1, \dots, \sequence'_m}}$,
where $\listIndex{\sequence}{\ell}$ is the index of input $\sequence$ in $\ell$.
\end{defi}

\begin{lem}
\label{theo:sublists}
    Let $\TestSuite$ be an input set and $\dataList{\sequence_1, \dots, \sequence_n}, \dataList{\sequence'_1, \dots, \sequence'_m}$ be two orders of removal steps in $\TestSuite$.
    If $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$ and $\dataList{\sequence'_1, \dots, \sequence'_m}$ is a \TSE{2.6}{subsequence} of $\dataList{\sequence_1, \dots, \sequence_n}$, then $\dataList{\sequence'_1, \dots, \sequence'_m} \in \ReducOrders{\TestSuite}$.
\end{lem}

\begin{proof}
The proof is done by induction on $m$.

If $m = 0$ then $\dataList{\sequence'_1, \dots, \sequence'_m} = \dataList{} \in \ReducOrders{\TestSuite}$.

Otherwise, we consider $\dataList{\sequence'_1, \dots, \sequence'_m, \sequence'_{m + 1}}$ and we assume by induction that $\dataList{\sequence'_1, \dots, \sequence'_m} \in \ReducOrders{\TestSuite}$.

Because $\dataList{\sequence'_1, \dots, \sequence'_m, \sequence'_{m + 1}}$ is a \TSE{2.6}{subsequence} of $\dataList{\sequence_1, \dots, \sequence_n}$, there exists an index $i$ such that $\sequence_i = \sequence'_{m + 1}$.
By definition of valid removal steps (\S III-C), % (\Cref{defi:validSteps}),
we have $\sequence_i \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}}{}}$.

Moreover, $\dataList{\sequence'_1, \dots, \sequence'_m, \sequence'_{m + 1}}$ is a \TSE{2.6}{subsequence} of $\dataList{\sequence_1, \dots, \sequence_i}$, so we have $\set{\sequence \in \dataList{\sequence'_1, \dots, \sequence'_m}}{} \subseteq \set{\sequence \in \dataList{\sequence_1, \dots, \sequence_{i - 1}}}{}$.
Hence, according to \Cref{theo:redundantReduction} we have $\Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}}{}} \subseteq \Redundant{\TestSuite \setminus \set{\sequence'_1, \dots, \sequence'_m}{}}$.
Therefore, $\sequence'_{m + 1} = \sequence_i \in \Redundant{\TestSuite \setminus \set{\sequence'_1, \dots, \sequence'_m}{}}$.

$\dataList{\sequence'_1, \dots, \sequence'_m} \in \ReducOrders{\TestSuite}$ and $\sequence'_{m + 1} \in \Redundant{\TestSuite \setminus \set{\sequence'_1, \dots, \sequence'_m}{}}$, so, according to our definition for valid orders of removal steps (\S III-C), % (\Cref{defi:validSteps}),
we have $\dataList{\sequence'_1, \dots, \sequence'_m, \sequence'_{m + 1}} \in \ReducOrders{\TestSuite}$.
\end{proof}

Finally, we prove in \Cref{theo:permutationValidOrder} that inputs in a valid order of removal steps can be rearranged in any different order and the rearranged order of removal steps is also valid.

\begin{lem}[Transposition of a Valid Order]
\label{theo:transpositionValidOrder}
    Let $\TestSuite$ be an input set.
    $$
    \begin{array}{r@{}l}
         \text{If } &  \dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite} \\
         \text{and } & 1 \le i < j \le n,
         \\[0.1cm]
         \text{then }& \dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \dots, \sequence_n} \in \ReducOrders{\TestSuite}
    \end{array}
    $$
    where $\sequence_i$ and $\sequence_j$ were exchanged and the other inputs are left unchanged.
    %In other words, $\transposition(\dataList{1, \dots, i, \dots, j, \dots, n}) = \dataList{1, \dots, j, \dots, i, \dots, n}$, where $\transposition = (ij)$ is the transposition exchanging $i$ and $j$.
\end{lem}

\begin{proof}
The proof is done in four steps.

1) $\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j}$ is a \TSE{2.6}{subsequence} of
$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$.
So, according to \Cref{theo:sublists}, we have $\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j} \in \ReducOrders{\TestSuite}$.
Note that the first step even applies to the case $i = 1$.

2) If $j = i + 1$, then one can go directly to the third step.
Otherwise, for each $i < k < j$, we denote:
$$
\begin{array}{l@{}l}
     \TestSuite_{i + 1}
        &\eqdef \TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}}{}  \\
     \TestSuite_{k + 1}
        &\eqdef \TestSuite_k \setminus \set{\sequence_k}{}
\end{array}
$$
and, for the sake of conciseness, $\TestSuite^i_k = \TestSuite_k \setminus \set{\sequence_i}{}$ and $\TestSuite^j_k = \TestSuite_k \setminus \set{\sequence_j}{}$.

We now prove by induction on $i \le k \le j - 1$ that:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_k} \in \ReducOrders{\TestSuite}$$

For the initialization $k = i$, we have from the first step:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j} \in \ReducOrders{\TestSuite}$$

We now assume by induction hypothesis on $i \le k < j - 1$ that:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_k} \in \ReducOrders{\TestSuite}$$

We first prove, for each $\actionSublass \in \getSubclasses{\sequence_{k + 1}}$, that:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}} > 1$$

According to \Cref{theo:orderWithoutRepetition}, $\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n$ are distinct.
We consider two cases.

a) We assume $\actionSublass \in \getSubclasses{\sequence_j}$.

Because $\TestSuite^i_j = \TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}, \sequence_i, \sequence_{i + 1}, \dots, \sequence_{j - 1}}{}$
and
$\TestSuite^j_{k + 1} = \TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}, \sequence_{i + 1}, \dots, \sequence_k, \sequence_j}{}$, we have $\TestSuite^i_j \cup \set{\sequence_{k + 1}}{} \subseteq \TestSuite^j_{k + 1} \cup \set{\sequence_j}{}$.
Thus, for each $\actionSublass \in \getSubclasses{\sequence_j} \cap \getSubclasses{\sequence_{k + 1}}$:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} + 1 \le \card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}} + 1$$

Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\redundancy{\sequence_j}{\TestSuite^i_j} > 0$$
So, for each $\actionSublass \in \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} > 1$$
Thus, for each $\actionSublass \in \getSubclasses{\sequence_j} \cap \getSubclasses{\sequence_{k + 1}}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}} > 1$$

b) We assume $\actionSublass \notin \getSubclasses{\sequence_j}$.

For each $\actionSublass \in \getSubclasses{\sequence_{k + 1}} \setminus \left(\getSubclasses{\sequence_i} \cup \getSubclasses{\sequence_j}\right)$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_{k + 1}} = \card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}}$$
Moreover, for each $\actionSublass \in \getSubclasses{\sequence_i} \setminus \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_{k + 1}} + 1 = \card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}}$$
So, for each $\actionSublass \in \getSubclasses{\sequence_{k + 1}} \setminus \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_{k + 1}} \le \card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}}$$
Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\redundancy{\sequence_{k + 1}}{\TestSuite^i_{k + 1}} > 0$$
So, for each $\actionSublass \in \getSubclasses{\sequence_{k + 1}}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_{k + 1}} > 1$$
Thus, for each $\actionSublass \in \getSubclasses{\sequence_{k + 1}} \setminus \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}} > 1$$

So, we proved by case, for each $\actionSublass \in \getSubclasses{\sequence_{k + 1}}$, that:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_{k + 1}} > 1$$

Thus, we have $\redundancy{\sequence_{k + 1}}{\TestSuite^j_{k + 1}} > 0$.

Moreover, according to \Cref{theo:orderWithoutRepetition}, $\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n$ are distinct, so $\sequence_{k + 1} \in \TestSuite^j_{k + 1}$.
Hence, $\sequence_{k + 1} \in \Redundant{\TestSuite^j_{k + 1}}$.
By induction hypothesis, we have:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_k} \in \ReducOrders{\TestSuite}$$

So, according to the definition of valid removal steps (\S III-C):  %\Cref{defi:validSteps}:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_k, \sequence_{k + 1}} \in \ReducOrders{\TestSuite}$$
which concludes the induction step.

Therefore, we proved by induction:
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_{j - 1}} \in \ReducOrders{\TestSuite}$$

3) We now prove that, for each $\actionSublass \in \getSubclasses{\sequence_i}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} > 1$$
where $\TestSuite^i_j$ and $\TestSuite^j_j$ are defined in step two.
We consider two cases.

a) We assume $\actionSublass \in \getSubclasses{\sequence_j}$.
Because $\TestSuite^i_j \cup \set{\sequence_i}{} = \TestSuite^j_j \cup \set{\sequence_j}{}$, for each $\actionSublass \in \getSubclasses{\sequence_i} \cap \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} + 1 = \card{\getSequences{\actionSublass} \cap \TestSuite^j_j} + 1$$

Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\redundancy{\sequence_j}{\TestSuite^i_j} > 0$$

So, for each $\actionSublass \in \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} > 1$$

Thus, for each $\actionSublass \in \getSubclasses{\sequence_i} \cap \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} > 1$$

b) We assume $\actionSublass \notin \getSubclasses{\sequence_j}$.
In that case, for each $\actionSublass \in \getSubclasses{\sequence_i} \setminus \getSubclasses{\sequence_j}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} + 1 = \card{\getSequences{\actionSublass} \cap \TestSuite^j_j}$$

We consider two cases.

i) There exists $i + 1 \le k \le j - 1$ such that $\actionSublass \in \getSubclasses{\sequence_k}$.
In that case, let $k_{\max}$ be the largest.
So, we have:
$$\left(\getSequences{\actionSublass} \cap \TestSuite^i_j\right) \cup \set{\sequence_{k_{\max}}}{} = \getSequences{\actionSublass} \cap \TestSuite^i_{k_{\max}}$$
Hence:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} + 1 = \card{\getSequences{\actionSublass} \cap \TestSuite^i_{k_{\max}}}$$
Thus:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} = \card{\getSequences{\actionSublass} \cap \TestSuite^i_{k_{\max}}}$$
Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\redundancy{\sequence_{k_{\max}}}{\TestSuite^i_{k_{\max}}} > 0$$
So, because $\actionSublass \in \getSubclasses{\sequence_{k_{\max}}}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_{k_{\max}}} > 1$$
Finally:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} > 1$$

ii) Otherwise, for each $i + 1 \le k \le j - 1$, we have $\actionSublass \notin \getSubclasses{\sequence_k}$.
Note that this is also the case if $j = i + 1$.
In that case, we have:
$$\left(\getSequences{\actionSublass} \cap \TestSuite^i_j\right) \cup \set{\sequence_i}{} = \getSequences{\actionSublass} \cap \TestSuite_i$$
where $\TestSuite_i = \TestSuite \setminus \set{\sequence_1, \dots, \sequence_{i - 1}}{}$.
So:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^i_j} + 1 = \card{\getSequences{\actionSublass} \cap \TestSuite_i}$$
Thus:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} = \card{\getSequences{\actionSublass} \cap \TestSuite_i}$$
Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\redundancy{\sequence_i}{\TestSuite_i} > 0$$
So, because $\actionSublass \in \getSubclasses{\sequence_i}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite_i} > 1$$
Finally:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} > 1$$

This concludes the proof by case for $\actionSublass \in \getSubclasses{\sequence_i} \setminus \getSubclasses{\sequence_j}$.
Therefore, we proved by case that, for each $\actionSublass \in \getSubclasses{\sequence_i}$, we have:
$$\card{\getSequences{\actionSublass} \cap \TestSuite^j_j} > 1$$

Thus, we have $\redundancy{\sequence_i}{\TestSuite^j_j} > 0$.

Moreover, according to \Cref{theo:orderWithoutRepetition}, $\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n$ are distinct, so $\sequence_i \in \TestSuite^j_j$.
Thus, $\sequence_i \in \Redundant{\TestSuite^j_j}$.

Finally, we have from the second step (or the first one, if $j = i + 1$):
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_{j - 1}} \in \ReducOrders{\TestSuite}$$

Therefore, according to the definition of valid orders of removal steps (\S III-C): % (\Cref{defi:validSteps}):
$$\dataList{\sequence_1, \dots, \sequence_{i - 1}, \sequence_j, \sequence_{i + 1}, \dots, \sequence_{j - 1}, \sequence_i} \in \ReducOrders{\TestSuite}$$

4) Finally, if $j = n$ then the proof is complete.
Otherwise, we prove by induction on $j \le k \le n$ that:
$$\dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \sequence_{j + 1}, \dots, \sequence_k} \in \ReducOrders{\TestSuite}$$

For the initialization $k = j$, we have from the third step:
$$\dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i} \in \ReducOrders{\TestSuite}$$

We now assume by induction hypothesis on $j \le k < n$ that:
$$\dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \sequence_{j + 1}, \dots, \sequence_k} \in \ReducOrders{\TestSuite}$$
Because $\dataList{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, we have:
$$\sequence_{k + 1} \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_k}{}}$$
Moreover, we have:
$$
\begin{array}{l}
\set{\sequence_1, \dots, \sequence_i, \dots, \sequence_j, \dots, \sequence_k}{}\\
= \set{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \dots, \sequence_k}{}
\end{array}
$$
So:
$$\sequence_{k + 1} \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \dots, \sequence_k}{}}$$
Thus, according to the definition of valid orders of removal steps  (\S III-C): % (\Cref{defi:validSteps}):
$$
\begin{array}{l}
\dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \sequence_{j + 1}, \dots, \sequence_k, \sequence_{k + 1}}\\
\in \ReducOrders{\TestSuite}
\end{array}
$$
which concludes the induction step.

Therefore, we proved by induction the \namecref{theo:transpositionValidOrder}:
$$\dataList{\sequence_1, \dots, \sequence_j, \dots, \sequence_i, \sequence_{j + 1}, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$$
\end{proof}

The issue with our definition of the gain (\S III-C) % (\Cref{defi:gainExhaust})
is that, to compute $\gainExhaust{\TestSuite}$ of an input set $\TestSuite$, one has to try all the possible order of removal steps to determine which ones are valid.
If $\TestSuite$ contains $n$ inputs and we consider orders of $0 \le k \le n$ removal steps, there are $n \times \dots \times (n - k + 1) = \frac{\factorial{n}}{\factorial{(n - k)}}$ possibilities to investigate, which is usually large.

Thus, we present an optimization to reduce the cost of computing the gain.
First, we prove in \Cref{theo:appendix:permutationValidOrder} that, while the order of inputs matters to determine if an order of removal steps is valid, it does not matter anymore once we know the order is valid.
In other words, inputs in a valid order of removal steps may be rearranged in any different order, and the rearranged order of removal steps would be valid.
Formally, if $\dataList{\sequence_1, \dots, \sequence_n}$ is a valid order of removal steps, then $\dataList{\sequence_{\permutation(1)}, \dots, \sequence_{\permutation(n)}}$ is also a valid order, when $\permutation$ denotes a permutation of the $n$ inputs, i.e., the same inputs but (potentially) in a different order:

\begin{prop}[Permutation of a Valid Order]
\label{theo:permutationValidOrder}
\label{theo:appendix:permutationValidOrder}
    Let $\TestSuite$ be an input set.
    If $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$ and $\permutation$ is a permutation on $n$ elements, then $\dataList{\sequence_{\permutation(1)}, \dots, \sequence_{\permutation(n)}} \in \ReducOrders{\TestSuite}$.
\end{prop}

\begin{proof}
Every permutation of a finite set can be expressed as the product of transpositions~\cite{Mar59} (p.60).
Let $m$ be the number of such transpositions for $\permutation$.
We prove the result by induction on $m$.

If $m = 0$, then $\permutation$ is the identity and we have by hypothesis:
$$\dataList{\sequence_{\permutation(1)}, \dots, \sequence_{\permutation(n)}} \in \ReducOrders{\TestSuite}$$

If $\permutation = \transposition_{m + 1} \circ \transposition_m \circ \dots \circ \transposition_1$, then we denote $\permutation' = \transposition_m \circ \dots \circ \transposition_1$.
By induction hypothesis, we have:
$$\dataList{\sequence_{\permutation'(1)}, \dots, \sequence_{\permutation'(n)}} \in \ReducOrders{\TestSuite}$$

Then, by applying \Cref{theo:transpositionValidOrder} to the transposition $(ij) = \transposition_{m + 1}$, we have:
$$\dataList{\sequence_{\transposition_{m + 1} \circ \permutation'(1)}, \dots, \sequence_{\transposition_{m + 1} \circ \permutation'(n)}} \in \ReducOrders{\TestSuite}$$

Finally, because $\permutation = \transposition_{m + 1} \circ \permutation'$, we conclude the induction step.
\end{proof}

\TSE{2.1}{Since inputs in a valid order of removal steps are always distinct (\Cref{theo:orderWithoutRepetition}) and their order does not make a difference (\Cref{theo:appendix:permutationValidOrder}), such orders can simply be seen as sets even if, in practice, for \impro and \geneticAlgo, orders of removal steps are implemented as lists.
More precisely, two valid orders of removal steps are equivalent if they correspond to the same set of inputs.
We leverage this property to reduce the number of orders of removal steps to consider, e.g., since $\dataList{\sequence_1, \sequence_2}$ is equivalent to $\dataList{\sequence_2, \sequence_1}$, we only have to check that $\dataList{\sequence_1, \sequence_2}$ is valid to know whether $\dataList{\sequence_2, \sequence_1}$ is valid or not.
This means that, when inputs are provided in a given order $\dataList{\sequence_1, \dots, \sequence_n}$, these tools need only to check for valid orders of removal steps in increasing order (hence without backtracking on previous inputs), i.e., $\dataList{\sequence_{i_1}, \dots, \sequence_{i_m}}$, where $1 \le i_1 < \dots < i_m \le n$.
We call \emph{canonical orders} such orders of removal steps.
For instance, $\dataList{\sequence_2, \sequence_4, \sequence_7}$ is in canonical order, but $\dataList{\sequence_4, \sequence_2, \sequence_7}$ is not.
Thus, to save time when checking the validity of orders of removal steps, we consider only canonical orders.
% In other words, when two orders of removal steps are equivalent, we consider the canonical order as the representative of the equivalence class.
}

\begin{theo}[Canonical Order]
\label{theo:canonicalOrder}
\label{theo:appendix:canonicalOrder}
    Let $\TestSuite = \set{\sequence_1, \dots, \sequence_n}{}$ be an input set.
    There exists $\dataList{\sequence_{i_1}, \dots, \sequence_{i_m}} \in \ReducOrders{\TestSuite}$ such that $1 \le i_1 < \dots < i_m \le n$ and:
    $$\sum_{1 \le j \le m} \costFunction{\sequence_{i_j}} = \gainExhaust{\TestSuite}$$
\end{theo}

\begin{proof}
Let $\dataList{\sequence_{i'_1}, \dots, \sequence_{i'_m}} \in \ReducOrders{\TestSuite}$ be a valid order of removal steps with a maximal cumulative cost i.e., according to our definition of the gain (\S III-C): %\Cref{defi:gainExhaust}:
$$\sum_{1 \le j \le m} \costFunction{\sequence_{i'_j}} = \gainExhaust{\TestSuite}$$

If $m = 0$, then $\dataList{}$ satisfies the \namecref{theo:canonicalOrder} for a gain $= 0$.

Otherwise, we assume $m > 0$.
According to \Cref{theo:orderWithoutRepetition}, $\dataList{\sequence_{i'_1}, \dots, \sequence_{i'_m}}$ contains $m$ distinct inputs.
Let $\permutation \in \symmetricGroup{m}$ be the permutation such that:
$$\dataList{\sequence_{\permutation(i'_1)}, \dots, \sequence_{\permutation(i'_m)}} = \dataList{\sequence_{i_1}, \dots, \sequence_{i_m}}$$
with $1 \le i_1 < \dots < i_m \le n$.

According to \Cref{theo:permutationValidOrder}, we have $\dataList{\sequence_{i_1}, \dots, \sequence_{i_m}} \in \ReducOrders{\TestSuite}$.

Moreover, because a permutation of the elements of a sum does not change the value of the sum, we have:
$$\sum_{1 \le j \le m} \costFunction{\sequence_{i_j}} = \sum_{1 \le j \le m} \costFunction{\sequence_{i'_j}} = \gainExhaust{\TestSuite}$$

Hence the \namecref{theo:canonicalOrder}.
\end{proof}

\Cref{theo:canonicalOrder} allows us to focus on inputs in increasing order, instead of exploring all possible input orders.
Thus, this optimization saves computation steps and makes computing the gain more tractable.
More precisely, since there are $\factorial{k}$ ways of ordering $k$ selected inputs, there are \quotes{only} $\frac{\factorial{n}}{\factorial{k}\factorial{(n - k)}}$ remaining possibilities to investigate, instead of $\frac{\factorial{n}}{\factorial{(n - k)}}$.


==> Appendices/proofs_search.tex <==
\section{Formal results for the Search}
%\label{sec:aim:appendix:search}


%%%%%%%%%%%%%%%%
\subsection{Local Dominance}
\label{sec:aim:appendix:localDominance}

In this section we prove, as presented in \S VII-E, %  \Cref{sec:aim:localDominance},
that the local dominance relation is local (\Cref{theo:local}), hence is faithful to its name, and that non locally-dominated inputs, as a whole, locally-dominate all the locally dominated inputs (\Cref{theo:localDomHierarchy}).
We start by the locality property.

\begin{prop}[Local Dominance is Local]
\label{theo:local}
\label{theo:appendix:local}
    Let $\sequence_1 \in \SearchSpace$ be a remaining input and $S \subseteq \SearchSpace$ be a subset of the remaining inputs.
    If $\sequence_1 \localDom S$ then $\sequence_1 \localDom S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}$.
\end{prop}

\begin{proof}
We assume $\sequence_1 \localDom S$.
So, by definition of local dominance (\S VII-E), % (\Cref{defi:localDominance}),
we have $\sequence_1 \not\in S$, $\getSubclasses{\sequence_1} \subseteq \getSubclasses{S}$, and $\costFunction{\sequence_1} \ge \costFunction{S}$.
First, because $\sequence_1 \not\in S$, we have $\sequence_1 \not\in S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}$.

Moreover, for every $\sequence_2 \in \SearchSpace$, if there is no overlap between $\sequence_1$ and $\sequence_2$ then, according to  the overlapping relation (\S VII-E), % (\Cref{defi:overlapRel}),
we have $\getSubclasses{\sequence_1} \cap \getSubclasses{\sequence_2} = \varnothing$.
Thus:
$$\getSubclasses{\sequence_1} \cap \getSubclasses{S \cap \set{\sequence_2 \in \SearchSpace}{\neg \sequence_1 \overlap \sequence_2}} = \varnothing$$
Hence, because $\getSubclasses{\sequence_1} \subseteq \getSubclasses{S}$, we have:
$$
\begin{array}{l}
    \getSubclasses{\sequence_1}
    {}\\
    = \getSubclasses{\sequence_1} \cap \getSubclasses{S} \\
    = \getSubclasses{\sequence_1} \cap (\getSubclasses{S\cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}\\
     \quad \cup\ \getSubclasses{S\cap \set{\sequence_2 \in \SearchSpace}{\neg \sequence_1 \overlap \sequence_2}})\\
     = (\getSubclasses{\sequence_1} \cap \getSubclasses{S\cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}) \\
     \quad \cup\ (\getSubclasses{\sequence_1}\\
     \quad \quad \cap\  \getSubclasses{S\cap \set{\sequence_2 \in \SearchSpace}{\neg \sequence_1 \overlap \sequence_2}}) \\
     = (\getSubclasses{\sequence_1} \cap \getSubclasses{S\cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}) \\
\end{array}
$$
So, $\getSubclasses{\sequence_1} \subseteq \getSubclasses{S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}$.

Finally, $\costFunction{S} \ge \costFunction{S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}$.
Thus, because $\costFunction{\sequence_1} \ge \costFunction{S}$, we have $\costFunction{\sequence_1} \ge \costFunction{S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}}$.

Therefore, $\sequence_1 \localDom S \cap \set{\sequence_2 \in \SearchSpace}{\sequence_1 \overlap \sequence_2}$.
\end{proof}

We now prove that the local dominance relation is asymmetric (\Cref{theo:partDomAsymmetry}).
First, because an input always covers some objectives, it can be locally dominated only by a non-empty input subset.

\begin{lem}[Non-Empty Local Dominance]
\label{theo:dominanceEmpty}
    Let $\sequence \in \SearchSpace$ be an input and $S \subseteq \SearchSpace$ be a subset of the remaining inputs.
    If $\sequence \localDom S$ then $S \neq \varnothing$.
\end{lem}

\begin{proof}
    The proof is done by contradiction.
    If $S = \varnothing$ then $\getSubclasses{S} = \varnothing$.
    Because $\sequence \localDom S$ we have $\getSubclasses{\sequence} \subseteq \getSubclasses{S}$.
    So, $\getSubclasses{\sequence} = \varnothing$, which contradicts \Cref{theo:SubclassesNotEmpty}.
\end{proof}

Second, when two inputs locally dominates each other, they are equi\-valent in the sense of the equivalence relation from \S VII-D (two inputs are equivalent if they have the same coverage and cost), % \Cref{defi:equivSeqs},
that we denote $\equivSeqs$ in the following.
But, because we removed duplicates in \S VII-D, % \Cref{sec:aim:duplicates},
this case can happen only if the inputs are the same, which is excluded by the definition of local dominance (\S VII-E). % \Cref{defi:localDominance}.

\begin{lem}[Local Dominance for Singletons is Asymmetric]
\label{theo:dominanceAntisymmetry}
    Let $\sequence_1, \sequence_2 \in \SearchSpace$ be two inputs.
    If $\sequence_1 \localDom \set{\sequence_2}{}$, then $\sequence_2 \not\localDom \set{\sequence_1}{}$.
\end{lem}

\begin{proof}
    We assume by contradiction that $\sequence_1 \localDom \set{\sequence_2}{}$ and $\sequence_2 \localDom \set{\sequence_1}{}$.
    
    Hence, we have:
    1)
    $\getSubclasses{\sequence_1} \subseteq \getSubclasses{\sequence_2}$ and $\getSubclasses{\sequence_2} \subseteq \getSubclasses{\sequence_1}$, so $\getSubclasses{\sequence_1} = \getSubclasses{\sequence_2}$.
    2)
    $\costFunction{\sequence_1} \ge \costFunction{\sequence_2}$ and $\costFunction{\sequence_2} \ge \costFunction{\sequence_1}$, so $\costFunction{\sequence_1} = \costFunction{\sequence_2}$.
    So, we have $\sequence_1 \equivSeqs \sequence_2$.
    
    Because we removed duplicates in \S VII-D, % \Cref{sec:aim:duplicates},
    we have $\sequence_1 = \sequence_2$.
    So, $\sequence_1 \localDom \set{\sequence_1}{}$, which contradicts in the definition of local dominance (\S VII-E) % \Cref{defi:localDominance} 
    that an input cannot locally dominates itself.
\end{proof}

Note that this result is also useful to prove transitivity (\Cref{theo:partDomTransitivity}).

Third, because the cost of an input is positive, if an input is locally dominated by several inputs, then they have a strictly smaller cost.

\begin{lem}[Cost Hierarchy]
\label{theo:costHierarch}
    Let $\sequence_1 \in \SearchSpace$ be an input and $S \subseteq \SearchSpace$ be a subset of the remaining inputs.
    If $\sequence_1 \localDom S$ and $\card{S} \ge 2$ then for every $\sequence_2 \in S$ we have $\costFunction{\sequence_2} < \costFunction{\sequence_1}$.
\end{lem}

\begin{proof}
    Because $\sequence_1 \localDom S$ we have $\costFunction{\sequence_1} \ge \costFunction{S}$.
    So, for every $\sequence_2 \in S$ we have $\costFunction{\sequence_2} \le \costFunction{\sequence_1}$.
    If $\card{S} \ge 2$, then the inequality is strict because, according to \Cref{theo:costPositive}, the cost is positive $\costFunction{\sequence_2} > 0$.
\end{proof}

Finally, we prove as expected that the local dominance relation is asymmetric.

\begin{prop}[Local Dominance for Subsets is Asymmetric]
\label{theo:dominanceAsymmetry}
    Let $\sequence_1, \sequence_2 \in \SearchSpace$ be two inputs and $S_1, S_2 \subseteq \SearchSpace$ be two subsets of the remaining inputs.
    If $\sequence_1 \localDom S_1$, $\sequence_2 \in S_1$, and $\sequence_2 \localDom S_2$, then $\sequence_1 \not\in S_2$.
\end{prop}

\begin{proof}
    The proof is made by contradiction.
    We assume $\sequence_1 \in S_2$ and prove a contradiction in different cases for $\card{S_1}$ and $\card{S_2}$.

    $\card{S_1} = 0$ or $\card{S_2} = 0$ are not possible, because this would contradict \Cref{theo:dominanceEmpty}.

    If $\card{S_1} = 1$ and $\card{S_2} = 1$, then $S_1 = \set{\sequence_2}{}$ and $S_2 = \set{\sequence_1}{}$.
    Thus, $\sequence_1 \localDom \set{\sequence_2}{}$ and $\sequence_2 \localDom \set{\sequence_1}{}$, which contradicts \Cref{theo:dominanceAntisymmetry}.

    If $\card{S_1} = 1$ then $S_1 = \set{\sequence_2}{}$.
    Because $\sequence_1 \localDom S_1$, we have $\costFunction{\sequence_1} \ge \costFunction{\sequence_2}$.
    Moreover, because $\sequence_2 \localDom S_2$ and $\sequence_1 \in S_2$, if $\card{S_2} \ge 2$ then according to \Cref{theo:costHierarch} we have $\costFunction{\sequence_1} < \costFunction{\sequence_2}$, hence the contradiction.

    Because $\sequence_1 \localDom S_1$ and $\sequence_2 \in S_1$, if $\card{S_1} \ge 2$ then according to \Cref{theo:costHierarch} we have $\costFunction{\sequence_2} < \costFunction{\sequence_1}$.
    Because $\sequence_2 \localDom S_2$ and $\sequence_1 \in S_2$, if $\card{S_2} \ge 2$ then according to \Cref{theo:costHierarch} we have $\costFunction{\sequence_1} < \costFunction{\sequence_2}$.
    Hence the contradiction $\costFunction{\sequence_1} < \costFunction{\sequence_1}$.
\end{proof}


Based on our definition of local dominance for subsets (\S VII-E), % (\Cref{defi:localDominance}),
we introduce the corresponding definition for inputs, in order to state more easily \Cref{theo:dominanceAcyclic}, then prove \Cref{theo:localDomHierarchy}.

\begin{defi}[Local Dominance]
\label{defi:localDominanceInputs}
    The input $\sequence_1 \in \SearchSpace$ \emph{locally-dominates} the input $\sequence_2 \in \SearchSpace$, denoted $\sequence_1 \partDom \sequence_2$, if there exists a subset $S \subseteq \SearchSpace$ such that $\sequence_1 \in S$ and $\sequence_2 \localDom S$.
\end{defi}

\begin{prop}[Local Dominance for Inputs is Asymmetric]
\label{theo:partDomAsymmetry}
\label{theo:appendix:partDomAsymmetry}
    The $\partDom$ relation is asymmetric i.e., for every $\sequence_1, \sequence_2\in \SearchSpace$, if $\sequence_2 \partDom \sequence_1$, then $\sequence_1 \not\partDom \sequence_2$.
\end{prop}

\begin{proof}
    If $\sequence_2 \partDom \sequence_1$ then there exists $S_1 \subseteq \SearchSpace$ such that $\sequence_2 \in S_1$ and $\sequence_1 \localDom S_1$.
    The proof is done by contradiction, assuming $\sequence_1 \partDom \sequence_2$.
    Hence, there exists $S_2 \subseteq \SearchSpace$ such that $\sequence_1 \in S_2$ and $\sequence_2 \localDom S_2$
    According to \Cref{theo:dominanceAsymmetry} we have $\sequence_1 \not\in S_2$, hence the contradiction.
\end{proof}

We now prove that the local dominance relation is transitive (\Cref{theo:partDomTransitivity}).

\begin{prop}[Local Dominance for Subsets is Transitive]
\label{theo:dominanceTransitive}
    Let $\sequence_1, \sequence_2 \in \SearchSpace$ be two inputs and $S_1, S_2 \subseteq \SearchSpace$ be two subsets of the remaining inputs.

    If $\sequence_1 \localDom S_1$, $\sequence_2 \in S_1$, and $\sequence_2 \localDom S_2$, then $\sequence_1 \localDom (S_1 \setminus \set{\sequence_2}{}) \cup S_2$.
\end{prop}

\begin{proof}
    Because $\getSubclasses{\sequence_1} \subseteq \getSubclasses{S_1}$, $\sequence_2 \in S_1$, and $\getSubclasses{\sequence_2} \subseteq \getSubclasses{S_2}$, we have:
    $$
    \begin{array}{r@{}l}
         \getSubclasses{\sequence_1}
            &{}\subseteq \getSubclasses{S_1 \setminus \set{\sequence_2}{}} \cup \getSubclasses{S_2}\\
            &{}= \getSubclasses{(S_1 \setminus \set{\sequence_2}{}) \cup S_2}
    \end{array}
    $$

    Moreover, because $\costFunction{\sequence_1} \ge \costFunction{S_1}$, $\sequence_2 \in S_1$, and $\costFunction{\sequence_2} \ge \costFunction{S_2}$, we have:
    $$
    \begin{array}{r@{}l}
         \costFunction{\sequence_1}
            &{}\ge \costFunction{S_1 \setminus \set{\sequence_2}{}} + \costFunction{S_2}  \\
            &{}\ge \costFunction{(S_1 \setminus \set{\sequence_2}{}) \cup S_2}
    \end{array}
    $$
    
    Finally, because $\sequence_1 \localDom S_1$ we have $\sequence_1 \not\in S_1$.
    We prove $\sequence_1 \not\in (S_1 \setminus \set{\sequence_2}{}) \cup S_2$ by contradiction.
    If $\sequence_1 \in (S_1 \setminus \set{\sequence_2}{}) \cup S_2$ then, because $\sequence_1 \not\in S_1$, we have $\sequence_1 \in S_2$.
    In that case, we have
    $$
    \begin{array}{l}
         \costFunction{\sequence_1}\\
            \ge \costFunction{S_1 \setminus \set{\sequence_2}{}} + \costFunction{S_2}\\
            = \costFunction{S_1 \setminus \set{\sequence_2}{}} + \costFunction{S_2 \setminus \set{\sequence_1}{}} + \costFunction{\sequence_1}\\
            \ge \costFunction{\sequence_1}
    \end{array}
    $$
    
    Hence, by subtracting $\costFunction{\sequence_1}$, we have:
    $$\costFunction{S_1 \setminus \set{\sequence_2}{}} + \costFunction{S_2 \setminus \set{\sequence_1}{}} = 0$$
    
    Thus, according to \Cref{theo:costPositive}, we have $S_1 = \set{\sequence_2}{}$ and $S_2 = \set{\sequence_1}{}$.
    Therefore $\sequence_1 \localDom \set{\sequence_2}{}$ and $\sequence_2 \localDom \set{\sequence_1}{}$, which contradicts \Cref{theo:dominanceAntisymmetry}.
\end{proof}

\begin{prop}[Local Dominance for Inputs is Transitive]
\label{theo:partDomTransitivity}
\label{theo:appendix:partDomTransitivity}
    The $\partDom$ relation is transitive i.e., for every $\sequence_1, \sequence_2, \sequence_3 \in \SearchSpace$, if $\sequence_3 \partDom \sequence_2$ and $\sequence_2 \partDom \sequence_1$, then $\sequence_3 \partDom \sequence_1$.
\end{prop}

\begin{proof}
    If $\sequence_3 \partDom \sequence_2$ and $\sequence_2 \partDom \sequence_1$, then there exists $S_1, S_2\subseteq \SearchSpace$ such that $\sequence_2 \in S_1$, $\sequence_1 \localDom S_1$, $\sequence_3 \in S_2$, and $\sequence_2 \localDom S_2$.
    According to \Cref{theo:dominanceTransitive}, we have $\sequence_1 \localDom (S_1 \setminus \set{\sequence_2}{}) \cup S_2$.
    Hence, because $\sequence_3 \in S_2 \subseteq (S_1 \setminus \set{\sequence_2}{}) \cup S_2$ we have $\sequence_3 \partDom \sequence_1$.
\end{proof}

We finally prove that the local dominance relation is acyclic.

\begin{cor}[Local Dominance is Acyclic]
\label{theo:dominanceAcyclic}
\label{theo:appendix:dominanceAcyclic}
    There exists no cycle $\sequence_1 \partDom \dots \partDom \sequence_n \partDom \sequence_1$ such that $\sequence_1, \dots, \sequence_n \in \SearchSpace$.
\end{cor}

\begin{proof}
    The proof is done by contradiction, by assuming the existence of such a cycle $\sequence_1 \partDom \dots \partDom \sequence_n \partDom \sequence_1$.
    According to \Cref {theo:partDomTransitivity}, we have by transitivity that $\sequence_1 \partDom \sequence_1$.
    Then, according to \Cref {theo:partDomAsymmetry}, we have by asymmetry $\sequence_1 \not\partDom \sequence_1$.
    Hence the contradiction.
\end{proof}

Finally, we use the transitivity (\Cref{theo:partDomTransitivity} and \Cref{theo:dominanceTransitive}) and the acycli\-city (\Cref{theo:dominanceAcyclic}) of the local-dominance relation to prove that non locally-dominated inputs, as a whole, locally-dominate all the locally dominated inputs.

\begin{theo}[Local Dominance Hierarchy]
\label{theo:localDomHierarchy}
\label{theo:appendix:localDomHierarchy}
    For every locally-dominated input $\sequence \in \SearchSpace$, there exists a subset $S \subseteq \SearchSpace$ of not locally-dominated inputs such that $\sequence \localDom S$.
\end{theo}

\begin{proof}
For each input $\sequence_0 \in \SearchSpace$ we denote:
$$\LocDoms{\sequence_0} \eqdef \set{\sequence \in \SearchSpace}{\sequence \partDom \sequence_0}$$
the input set which locally dominate $\sequence_0$.

Let $\sequence_0 \in \SearchSpace$ be an input.
We prove by induction on $\LocDoms{\sequence_0}$ that either $\sequence_0$ is not locally dominated or there exists a subset $S \subseteq \SearchSpace$ of not locally-dominated inputs such that $\sequence_0 \localDom S$.

For the initialization, we consider $\LocDoms{\sequence_0} = \varnothing$.
In that case, $\sequence_0$ is not locally dominated.

For the induction step, we consider $\LocDoms{\sequence_0} \neq \varnothing$, so $\sequence_0$ is a locally dominated input.
Hence, there exists $S_0 \subseteq \SearchSpace$ such that $\sequence_0 \localDom S_0$.
We consider two cases.

Either every input in $S_0$ is not locally dominated.
In that case $S = S_0$ satisfies the inductive property.

Or there exists $n \ge 1$ input $\sequence_1, \dots, \sequence_n$ in $S_0$ which are locally dominated.
The rest of the proof is done in two steps.

First, let $1 \le i \le n$.
We prove that $\LocDoms{\sequence_i} \subset \LocDoms{\sequence_0}$, with a strict inclusion.

Because $\sequence_i \in S_0$ and $\sequence_0 \localDom S_0$, we have $\sequence_i \partDom \sequence_0$.
Hence, $\sequence_i \in \LocDoms{\sequence_0}$.

Let $\sequence \in \LocDoms{\sequence_i}$, so we have $\sequence \partDom \sequence_i$.
So, according to \Cref{theo:partDomTransitivity}, we have by transitivity $\sequence \partDom \sequence_0$, thus $\sequence \in \LocDoms{\sequence_0}$.
Hence, $\LocDoms{\sequence_i} \subseteq \LocDoms{\sequence_0}$.

According to \Cref{theo:dominanceAcyclic}, there is no cycle so $\sequence_i \not\partDom \sequence_i$.
Hence, $\sequence_i \not\in \LocDoms{\sequence_i}$.

Finally, we have $\LocDoms{\sequence_i} \subseteq \LocDoms{\sequence_0}$ and $\sequence_i \in \LocDoms{\sequence_0} \setminus \LocDoms{\sequence_i}$.
Therefore $\LocDoms{\sequence_i} \subset \LocDoms{\sequence_0}$.

Because $\LocDoms{\sequence_i} \subset \LocDoms{\sequence_0}$, we can apply the induction hypothesis on $\sequence_i$, which is locally dominated.
Therefore, for each $1 \le i \le n$, there exists a subset $S_i \subseteq \SearchSpace$ of not locally-dominated inputs such that $\sequence_i \localDom S_i$.

Second, we use these $S_i$ to define by induction on $0 \le m < n$ the following input sets:
$$
\begin{array}{l@{}l}
     \TestSuite_0
        &{}= S_0\\
     \TestSuite_{m + 1}
        &{}= (\TestSuite_m \setminus \set{\sequence_{m + 1}}{}) \cup S_{m + 1}
\end{array}
$$
and we prove by induction on $0 \le m \le n$ that $\sequence_0 \localDom \TestSuite_m$ and that
either, $m < n$ and $\sequence_{m + 1}, \dots, \sequence_n$ are the only locally dominated inputs in $\TestSuite_m$, or $m = n$ and $\TestSuite_m$ contains no locally dominated input.

For the initialization, we have $\TestSuite_0 = S_0$ and the inductive property is satisfied because $\sequence_0 \localDom S_0$ and $\sequence_1, \dots, \sequence_n$ are the only locally dominated inputs in $S_0$.

For the induction step $m + 1 \le n$, we assume that $\sequence_0 \localDom \TestSuite_m$ and that $\sequence_{m + 1}, \dots, \sequence_n$ are the only locally dominated inputs in $\TestSuite_m$.

Because $\TestSuite_{m + 1} = (\TestSuite_m \setminus \set{\sequence_{m + 1}}{}) \cup S_{m + 1}$ and $S_{m + 1}$ contains no locally-dominated input, we have that either, $m + 1 < n$ and $\sequence_{m + 2}, \dots, \sequence_n$ are the only locally dominated inputs in $\TestSuite_{m + 1}$, or $m + 1 = n$ and $\TestSuite_{m + 1}$ contains no locally-dominated input.

Moreover, because $\sequence_0 \localDom \TestSuite_m$, $\sequence_{m + 1} \in \TestSuite_m$, and $\sequence_{m + 1} \localDom S_{m + 1}$, then according to \Cref{theo:dominanceTransitive}, we have $\sequence_0 \localDom (\TestSuite_m \setminus \set{\sequence_{m + 1}}{}) \cup S_{m + 1}$.
Hence $\sequence_0 \localDom \TestSuite_{m + 1}$, which concludes the induction step.

Therefore, $\sequence_0 \localDom \TestSuite_n$ and $\TestSuite_n$ contains no locally-dominated input.
Thus, $S = \TestSuite_n$ satisfies the inductive property on $\LocDoms{\sequence_0}$.
Hence the claim for not locally-dominated inputs.
\end{proof}


%%%%%%%%%%%%%%%%
\subsection{Dividing the Problem}
\label{sec:aim:appendix:subproblem}

In this section, we prove that redundancy updates are local (\Cref{theo:localRedundancyUpdate}), that reductions on different connected components can be performed independently (\Cref{theo:redundantComps}), and finally that the gain can be independently computed on each connected component (\Cref{theo:splitExhaust}).
The main purpose of the section is to justify we can divide our problem into subproblems (\S VII-F). % (\Cref{defi:subprob}).
We start by the locality.

\begin{lem}[Redundancy Updates are Local]
\label{theo:localRedundancyUpdate}
\label{theo:appendix:localRedundancyUpdate}
    Let $\TestSuite$ be an input set and let $\sequence_1, \sequence_2 \in \TestSuite$.
    
    If $\redundancy{\sequence_2}{\TestSuite \setminus \set{\sequence_1}{}} \neq \redundancy{\sequence_2}{\TestSuite}$, then $\sequence_1 \overlap \sequence_2$.
\end{lem}

\begin{proof}
The proof is done by contraposition.
If $\sequence_1$ and $\sequence_2$ do not overlap, then $\getSubclasses{\sequence_1} \cap \getSubclasses{\sequence_2} = \varnothing$.
So, for every $\actionSublass \in \getSubclasses{\sequence_2}$, we have $\sequence_1 \not\in \getSequences{\actionSublass}$, and thus $\getSequences{\actionSublass} \cap (\TestSuite \setminus \set{\sequence_1}{}) = \getSequences{\actionSublass} \cap \TestSuite$.
Therefore, $\redundancy{\sequence_2}{\TestSuite \setminus \set{\sequence_1}{}} = \redundancy{\sequence_2}{\TestSuite}$.
\end{proof}

Then, we prove the independence of removal steps performed on different components.

\begin{lem}[Independent Redundancies]
\label{theo:independenceRedComps}
    Let $\TestSuite$ be an input set.
    For each connected component $\RedComp \in \RedundantComponents{\TestSuite}$, for each input $\sequence_0 \in \RedComp$, and for each order of removal steps $\dataList{\sequence_1, \dots, \sequence_n}$, if $\sequence_1, \dots, \sequence_n \not\in \RedComp$, then $\redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} = \redundancy{\sequence_0}{\TestSuite}$.
\end{lem}

\begin{proof}
$\RedundantComponents{\TestSuite}$ are the connected components for the redundant inputs in $\TestSuite$, hence they are disjoint.
Therefore, for each $\sequence_0 \in \RedComp$, because $\sequence_1, \dots, \sequence_n \not\in \RedComp$, we have that $\sequence_0$ do not overlap with any of the $\sequence_1, \dots, \sequence_n$.
Therefore, according to \Cref{theo:localRedundancyUpdate}, we have
$\redundancy{\sequence_0}{\TestSuite} = \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1}{}} = \dots = \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}$.
\end{proof}

\begin{prop}[Independent Removal Steps]
\label{theo:redundantComps}
\label{theo:appendix:redundantComps}
\hspace{0cm}

Let $\TestSuite$ be an input set and let $\RedComp_1, \dots, \RedComp_c \in \RedundantComponents{\TestSuite}$ denote $c$ connected components.
If, for each $0 \le i \le c$, there exists inputs $\sequence^i_1, \dots, \sequence^i_{n_i} \in \RedComp_i$ such that $\dataList{\sequence^i_1, \dots, \sequence^i_{n_i}} \in \ReducOrders{\TestSuite}$, then:
$$\dataList{\sequence^1_1, \dots, \sequence^1_{n_1}} + \dots + \dataList{\sequence^c_1, \dots, \sequence^c_{n_c}} \in \ReducOrders{\TestSuite}$$
where $+$ denotes \TSE{2.6}{sequence} concatenation.
\end{prop}

\begin{proof}
The proof is done by induction on $c$.

If $c = 0$, then $\dataList{\sequence^1_1, \dots, \sequence^1_{n_1}} + \dots + \dataList{\sequence^c_1, \dots, \sequence^c_{n_c}} = \dataList{} \in \ReducOrders{\TestSuite}$.

We assume by induction that $\dataList{\sequence^1_1, \dots, \sequence^1_{n_1}} + \dots + \dataList{\sequence^c_1, \dots, \sequence^c_{n_c}} \in \ReducOrders{\TestSuite}$.

We denote $\ell$ this order of removal steps and for the sake of simplicity we also denote $S = \set{\sequence^1_1, \dots, \sequence^1_{n_1}, \dots, \sequence^c_1, \dots, \sequence^c_{n_c}}{}$.

By induction, let $\RedComp_{c + 1} \in \RedundantComponents{\TestSuite}$ be another connected component and let $\sequence^{c + 1}_1$, \dots, $\sequence^{c + 1}_{n_{c + 1}} \in \RedComp_{c + 1}$ such that $\dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{n_{c + 1}}} \in \ReducOrders{\TestSuite}$.

We now prove that $\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{n_{c + 1}}} \in \ReducOrders{\TestSuite}$.

This is done by proving by induction on $0 \le j \le n_{c + 1}$ that:
$$\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_j} \in \ReducOrders{\TestSuite}$$
and that, for each $\sequence_0 \in \RedComp_{c + 1} \setminus S_j$, we have:
$$\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_j)} = \redundancy{\sequence_0}{\TestSuite \setminus S_j}$$
where $S_j = \set{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_j}{}$.

If $n_{c + 1} = 0$, then $\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{n_{c + 1}}} = \ell \in \ReducOrders{\TestSuite}$.
Moreover, because $\RedComp_{c + 1}$ is disjoint with $\RedComp_1, \dots, \RedComp_c$, according to \Cref{theo:independenceRedComps}, performing the $\ell$ removal steps does not change the redundancies of inputs in $\RedComp_{c + 1}$ i.e., for each $\sequence_0 \in \RedComp_{c + 1}$, we have $\redundancy{\sequence_0}{\TestSuite \setminus S} = \redundancy{\sequence_0}{\TestSuite}$.

We now assume by induction that $\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_j} \in \ReducOrders{\TestSuite}$ and for each $\sequence_0 \in \RedComp_{c + 1} \setminus S_j$, we have $\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_j)} = \redundancy{\sequence_0}{\TestSuite \setminus S_j}$.

Because $\dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{n_{c + 1}}} \in \ReducOrders{\TestSuite}$, we have $\sequence^{c + 1}_{j + 1} \in \Redundant{\TestSuite \setminus S_j}$.
Moreover, $\sequence^{c + 1}_{j + 1} \in \RedComp_{c + 1}$ hence $\sequence^{c + 1}_{j + 1} \not\in S$.
Therefore, using the induction hypothesis with $\sequence_0 = \sequence^{c + 1}_{j + 1}$, we have $\sequence^{c + 1}_{j + 1} \in \Redundant{\TestSuite \setminus (S \cup S_j)}$.
Therefore, according to our definition of valid removal steps (\S III-C), % (\Cref{defi:validSteps}),
$\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{j + 1}} \in \ReducOrders{\TestSuite}$.

We denote $S_{j + 1} = S_j \cup \set{\sequence^{c + 1}_{j + 1}}{}$.
Let $\sequence_0 \in \RedComp_{c + 1} \setminus S_{j + 1}$.

To complete the induction step, we prove that:
$$
\begin{array}{l}
\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_{j + 1})}\\
= \redundancy{\sequence_0}{\TestSuite \setminus S_{j + 1}}
\end{array}
$$

We remind that, for each input set $X$, we have:
$$
\begin{array}{l}
\redundancy{\sequence_0}{X}\\
= \min \set{\card{\getSequences{\actionSublass} \cap X}}{\actionSublass \in \getSubclasses{\sequence_0}} - 1
\end{array}
$$
We denote as critical the objectives contributing to the redundancy:
$$
\begin{array}{l}
\CriticalSubclasses{\sequence_0}{X}\\
\eqdef \arg \min \set{\card{\getSequences{\actionSublass} \cap X}}{\actionSublass \in \getSubclasses{\sequence_0}}
\end{array}
$$

Because $\sequence_0 \in \RedComp_{c + 1}$, we know that $\sequence_0$ does not overlap with inputs in $S$ so, for each $\actionSublass \in \getSubclasses{\sequence_0}$, we have $\getSequences{\actionSublass} \cap (\TestSuite \setminus S) = \getSequences{\actionSublass} \cap \TestSuite$.
Thus, by removing inputs of $S_j$ from both sides, we have $\getSequences{\actionSublass} \cap (\TestSuite \setminus (S \cup S_j)) = \getSequences{\actionSublass} \cap (\TestSuite \setminus S_j)$.
Therefore:
$$\CriticalSubclasses{\sequence_0}{\TestSuite \setminus (S \cup S_j)} = \CriticalSubclasses{\sequence_0}{\TestSuite \setminus S_j}$$

We consider two cases:

1) Either there exists $\actionSublass \in \CriticalSubclasses{\sequence_0}{\TestSuite \setminus S_j}$ such that $\sequence^{c + 1}_{j + 1} \in \getSequences{\actionSublass}$.
In that case:
$$
\begin{array}{l}
\card{\getSequences{\actionSublass} \cap (\TestSuite \setminus (S \cup S_{j + 1}))}\\
= \card{\getSequences{\actionSublass} \cap (\TestSuite \setminus (S \cup S_j))} - 1
\end{array}
$$
$$\card{\getSequences{\actionSublass} \cap (\TestSuite \setminus S_{j + 1})} = \card{\getSequences{\actionSublass} \cap (\TestSuite \setminus S_j)} - 1$$
Because $\actionSublass$ is critical and a redundancy can decrease at most by $1$ after a reduction (\Cref{theo:removingSeq}) so the cardinalities for other objectives cannot decrease below the previous redundancy minus one, we have:
$$
\begin{array}{l}
\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_{j + 1})}\\
= \redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_j)} - 1
\end{array}
$$
$$\redundancy{\sequence_0}{\TestSuite \setminus S_{j + 1}} = \redundancy{\sequence_0}{\TestSuite \setminus S_j} - 1$$

2) Or for each $\actionSublass \in \CriticalSubclasses{\sequence_0}{\TestSuite \setminus S_j}$, we have $\sequence^{c + 1}_{j + 1} \not\in \getSequences{\actionSublass}$.
In that case:
$$
\begin{array}{l}
\card{\getSequences{\actionSublass} \cap (\TestSuite \setminus (S \cup S_{j + 1}))}\\
= \card{\getSequences{\actionSublass} \cap (\TestSuite \setminus (S \cup S_j))}
\end{array}
$$
$$\card{\getSequences{\actionSublass} \cap (\TestSuite \setminus S_{j + 1})} = \card{\getSequences{\actionSublass} \cap (\TestSuite \setminus S_j)}$$
Because $\actionSublass$ is critical and a redundancy can decrease at most by $1$ after a reduction (\Cref{theo:removingSeq}) so the cardinalities for non-critical objectives cannot decrease below the previous redundancy we have:
$$
\begin{array}{l}
\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_{j + 1})}\\
= \redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_j)}
\end{array}
$$
$$\redundancy{\sequence_0}{\TestSuite \setminus S_{j + 1}} = \redundancy{\sequence_0}{\TestSuite \setminus S_j}$$

In both cases, by induction hypothesis $\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_j)} = \redundancy{\sequence_0}{\TestSuite \setminus S_j}$, hence we have $\redundancy{\sequence_0}{\TestSuite \setminus (S \cup S_{j + 1})} = \redundancy{\sequence_0}{\TestSuite \setminus S_{j + 1}}$.

This completes the induction on $0 \le j \le n_{c + 1}$.
In particular, we proved that $\ell + \dataList{\sequence^{c + 1}_1, \dots, \sequence^{c + 1}_{n_{c + 1}}} \in \ReducOrders{\TestSuite}$, which completes the induction on $c$, hence the result.
\end{proof}

We now prove that the gain can be independently computed on each connected component (\Cref{theo:splitExhaust}).
To do so, we have to prove intermediate results, including \Cref{theo:reducComponent}.

\begin{lem}[Redundancy within a connected component]
\label{theo:redundancyInComponent}
    Let $\TestSuite$ be an input set.
    For each connected component $\RedComp \in \RedundantComponents{\TestSuite}$, for each input $\sequence_0 \in \RedComp$, and for each order of removal steps $\dataList{\sequence_1, \dots, \sequence_n}$, if $\sequence_1, \dots, \sequence_n \in \RedComp$, then:
    $$
    \begin{array}{l}
     \redundancy{\sequence_0}{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}\\
     = \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}} 
    \end{array}
    $$
\end{lem}

\begin{proof}
We remind that, for each input set $X$, we have:
$$
\begin{array}{l}
\redundancy{\sequence_0}{X} \\
= \min \set{\card{\getSequences{\actionSublass} \cap X}}{\actionSublass \in \getSubclasses{\sequence_0}} - 1
\end{array}
$$

For the sake of simplicity, we denote $X_{\RedComp} = \RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}$ and $X_{\TestSuite} = \TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}$.
Let $\sequence_0 \in \RedComp$ and $\actionSublass \in \getSubclasses{\sequence_0}$.

Because $\RedComp \in \RedundantComponents{\TestSuite}$, we have $\RedComp \subseteq \TestSuite$, hence $X_{\RedComp} \subseteq X_{\TestSuite}$.
So $\getSequences{\actionSublass} \cap X_{\RedComp} \subseteq \getSequences{\actionSublass} \cap X_{\TestSuite}$.
Moreover, for each $\sequence \in \getSequences{\actionSublass} \cap X_{\TestSuite}$ we have $\actionSublass \in \getSubclasses{\sequence_0} \cap \getSubclasses{\sequence}$, so $\sequence_0 \overlap \sequence$, and thus $\sequence \in X_{\RedComp}$.

Therefore, $\getSequences{\actionSublass} \cap X_{\RedComp} = \getSequences{\actionSublass} \cap X_{\TestSuite}$.

Hence the result $\redundancy{\sequence_0}{X_{\RedComp}} = \redundancy{\sequence_0}{X_{\TestSuite}}$.
\end{proof}

\begin{cor}[Component Validity]
\label{theo:componentValidity}
    Let $\TestSuite$ be an input set.
    For each connected component $\RedComp \in \RedundantComponents{\TestSuite}$ and for each order of removal steps $\dataList{\sequence_1, \dots, \sequence_n}$, if $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\RedComp}$, then $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$.
\end{cor}

\begin{proof}
The proof is done by induction on $n$.

For the initialization $n = 0$, we have $\dataList{\sequence_1, \dots, \sequence_n} = \dataList{} \in \ReducOrders{\TestSuite}$.

For the induction step, we consider $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\RedComp}$ and we assume by induction that $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$.

Because $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\RedComp}$, according to our definition of redundant inputs and removal steps (\S III-C), % (\Cref{defi:redundantSeq,defi:validSteps}),
we have  $\sequence_1, \dots, \sequence_n \in \RedComp$.
Hence, according to \Cref{theo:redundancyInComponent}, we have for each $\sequence_0 \in \RedComp$:
$$
\begin{array}{l}
\redundancy{\sequence_0}{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}\\
= \redundancy{\sequence_0}{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}
\end{array}
$$

Thus, because $\RedComp \subseteq \TestSuite$, according to the definition of redundancy (\S III-C) % \Cref{defi:redundantSeq}
we have:
$$
\begin{array}{l}
\Redundant{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}\\
\subseteq \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}
\end{array}
$$

Because $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\RedComp}$, we have $\sequence_{n + 1} \in \Redundant{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}$ by definition of removal steps (\S III-C). % (\Cref{defi:validSteps}).
Thus, $\sequence_{n + 1} \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}$.

By induction hypothesis $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$.

Therefore %(\Cref{defi:validSteps}), we have 
$\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\TestSuite}$, which completes the induction step.
\end{proof}

\begin{prop}[Reductions withing a connected component]
\label{theo:reducComponent}
    Let $\TestSuite$ be an input set.
    For each connected component $\RedComp \in \RedundantComponents{\TestSuite}$ and for each order of removal steps $\dataList{\sequence_1, \dots, \sequence_n}$, if $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$ and $\sequence_1, \dots, \sequence_n \in \RedComp$, then $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\RedComp}$.
\end{prop}

\begin{proof}
The proof is done by induction on $n$.

If $n = 0$ then $\dataList{\sequence_1, \dots, \sequence_n} = \dataList{} \in \ReducOrders{\RedComp}$.

Otherwise, we consider $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}}$ with $\sequence_1, \dots, \sequence_n, \sequence_{n + 1} \in \RedComp$ and we assume by induction that $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\RedComp}$.

We assume $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\TestSuite}$, so $\sequence_{n + 1} \in \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}$.

According to \Cref{theo:redundancyInComponent} applied to inputs $\sequence_0 \in \RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}$ with redundancy $> 0$, we have:
$$
\begin{array}{l}
\Redundant{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}\\
= \Redundant{\TestSuite \setminus \set{\sequence_1, \dots, \sequence_n}{}}
\end{array}
$$

Hence, $\sequence_{n + 1} \in \Redundant{\RedComp \setminus \set{\sequence_1, \dots, \sequence_n}{}}$.

Thus, because $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\RedComp}$, according to our definition of valid removal steps (\S III-C), % (\Cref{defi:validSteps}),
we have the result $\dataList{\sequence_1, \dots, \sequence_n, \sequence_{n + 1}} \in \ReducOrders{\RedComp}$.
\end{proof}

Finally, we conclude the section by proving the claim on \Cref{theo:splitExhaust}, which is used to divide our problem into subproblems (\S VII-F). % (\Cref{defi:subprob}).

\begin{theo}[Divide the Gain]
    \label{theo:splitExhaust}\label{theo:appendix:splitExhaust}
    For each input set $\TestSuite$:
    $$\gainExhaust{\TestSuite} = \sum_{\RedComp \in \RedundantComponents{\TestSuite}} \gainExhaust{\RedComp}$$
\end{theo}

\begin{proof}
Let $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$ be a valid order of removal steps such that its cumulative cost $\sum_{1 \le i \le n} \costFunction{\sequence_i} = \gainExhaust{\TestSuite}$ is maximal (\S III-C), % (\Cref{defi:gainExhaust}),
and let $\RedundantComponents{\TestSuite} = \set{\RedComp_1, \dots, \RedComp_c}{}$ denote the connected components, without a particular order.

We denote $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_j}$ the largest sublist (\Cref{defi:sublists}) of $\dataList{\sequence_1, \dots, \sequence_n}$ contai\-ning only inputs in the connected component $\RedComp_j$.
Because $\dataList{\sequence_1, \dots, \sequence_n} \in \ReducOrders{\TestSuite}$, according to \Cref{theo:sublists} we have $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_j} \in \ReducOrders{\TestSuite}$ as well.
So, according to \Cref{theo:redundantComps}:
$$\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{1}} + \dots + \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{c}} \in \ReducOrders{\TestSuite}$$

Because the connected components form a partition of the redundant inputs, the cumulative cost of this order of removal steps is the same as $\dataList{\sequence_1, \dots, \sequence_n}$:
$$\sum_{1 \le j \le c} \sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j}}} \costFunction{\sequence} = \sum_{1 \le i \le n} \costFunction{\sequence_i} = \gainExhaust{\TestSuite}$$

We now consider any connected component $\RedComp_{j_1}$ and we prove that:
$$\sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}}} \costFunction{\sequence} = \gainExhaust{\RedComp_{j_1}}$$

The proof is done in two steps.

First, note that because $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}} \in \ReducOrders{\TestSuite}$ and contains only inputs in $\RedComp_{j_1}$, according to \Cref{theo:reducComponent} we have $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}} \in \ReducOrders{\RedComp_{j_1}}$ as well.

Second, we prove by contradiction that $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}}$ has a maximal cumulative cost in $\RedComp_{j_1}$.
We assume by contradiction that there exists a valid order of removal steps $\dataList{\sequence'_1, \dots, \sequence'_{n'}} \in \ReducOrders{\RedComp_{j_1}}$ such that:
$$\sum_{\sequence \in \dataList{\sequence'_1, \dots, \sequence'_{n'}}} \costFunction{\sequence} > \sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}}} \costFunction{\sequence}$$

Because $\dataList{\sequence'_1, \dots, \sequence'_{n'}} \in \ReducOrders{\RedComp_{j_1}}$, according to \Cref{theo:componentValidity} we have $\dataList{\sequence'_1, \dots, \sequence'_{n'}} \in \ReducOrders{\TestSuite}$ as well.
So, according to \Cref{theo:redundantComps}, we have:
$$\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{1}} + \dots + \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1 - 1}}$$
$$+ \dataList{\sequence'_1, \dots, \sequence'_{n'}} + \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1 + 1}} + \dots$$
$$+ \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{c}} \in \ReducOrders{\TestSuite}$$

The cumulative cost of this valid order of removal steps is thus larger than the cumulative cost of $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{1}} + \dots + \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{c}}$:
$$\sum_{\sequence \in \dataList{\sequence'_1, \dots, \sequence'_{n'}}} \costFunction{\sequence} + \sum_{1 \le j \le c \land j \neq j_1} \sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j}}} \costFunction{\sequence}$$
$$> \sum_{1 \le j \le c} \sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j}}} \costFunction{\sequence} = \gainExhaust{\TestSuite}$$
which contradicts the maximality of $\gainExhaust{\TestSuite}$.

Hence, $\dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}} \in \ReducOrders{\RedComp_{j_1}}$ has a maximal cumulative cost in $\RedComp_{j_1}$.
So, according to the definition of the gain (\S III-C), % (\Cref{defi:gainExhaust}),
we have for any connected component $\RedComp_{j_1}$:
$$\sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j_1}}} \costFunction{\sequence} = \gainExhaust{\RedComp_{j_1}}$$

Therefore, we have the result:
$$\gainExhaust{\TestSuite}
= \sum_{1 \le j \le c} \sum_{\sequence \in \dataList{\sequence_1, \dots, \sequence_n}_{\RedComp_{j}}} \costFunction{\sequence}
= \sum_{1 \le j \le c} \gainExhaust{\RedComp_j}$$
\end{proof}


%%%%%%%%%%%%%%%%
\subsection{Genetic Search}
\label{sec:aim:appendix:genetic}

In this section, we prove desirable properties satisfied for each generation by roofers (\Cref{theo:roofers}) and misers (\Cref{theo:misers}) during the genetic search (Section VIII). % (\Cref{sec:aim:genetic}).
We start by roofers.

\begin{theo}[Invariant of the Roofers]
\label{theo:roofers}
\label{theo:appendix:roofers}
    For every generation $n$, we have:
    $$\card{\Roofers{n}} = \sizePop$$
    $$
    \begin{array}{l}
    \min \set{\costFunction{\TestSuite}}{\TestSuite \in \Roofers{n}}\\
    = \min \set{\costFunction{\TestSuite}}{\TestSuite \in \bigcup\limits_{0 \le m \le n} \Roofers{m}}
    \end{array}
    $$
    and for every $\TestSuite \in \Roofers{n}$, we have:
    \begin{itemize}
        \item $\TestSuite$ is reduced (in the sense of \S III-C) % \Cref{defi:reduction})
        \item $\getSubclasses{\TestSuite} = \Objectives(\RedComp)$
    \end{itemize}
\end{theo}

\begin{proof}
There are $\sizePop$ individuals in the initial roofer population (\S VIII-B). % (\Cref{sec:aim:initPops}).
Moreover, the procedure detailed above to update the roofer population ensures that an offspring can only take the place of an existing roofer.
Hence, the number of roofers does not change over generations.

In the initial population, a roofer $\TestSuite$ is always replaced by its reduced counterpart $\reduction{\TestSuite}$ after adding an input (\S VIII-B). % (\Cref{sec:aim:initPops}).
Moreover, after mutation (\S VIII-E) % (\Cref{sec:aim:mutation})
each offspring $\TestSuite$ is replaced by its reduced counterpart $\reduction{\TestSuite}$ before determining if it is accepted in the roofer population or rejected.
Hence, for each generation, each roofer is reduced.

Roofers in the initial population are built so that they cover all the objectives (\S VIII-B). % (\Cref{sec:aim:initPops}).
Moreover, in the above procedure, an offspring can be added to the roofer population only if it covers all the objectives.
Hence, for each generation, each roofer covers all the objectives.

Finally, in the above procedure one can remove an individual from the roofer population only if a less or equally costly roofer is found.
Hence, the minimal cost amongst the roofers can only remain the same or decrease over generations.
Therefore, the minimal cost in the last generation is the minimal cost encountered so far during the search.
\end{proof}

To ease the proof for misers (\Cref{theo:misers}), we first prove in \Cref{theo:miserDom} that a miser $\TestSuite_0$ can be removed between generation $n$ and generation $n + 1$ only by a dominating miser $\TestSuite$.
Then, we prove in \Cref{theo:miserTemporalDom} that being dominated is carried from generation to generation.

\begin{lem}[Transitivity of Pareto Dominance]
\label{theo:ParetoDomTransitive}
    The $\dominates$ relation (\S II-E) % (\Cref{defi:pareto})
    is transitive i.e., for every input sets $\TestSuite_1, \TestSuite_2, \TestSuite_3$, if $\TestSuite_1 \dominates \TestSuite_2$ and $\TestSuite_2 \dominates \TestSuite_3$, then $\TestSuite_1 \dominates \TestSuite_3$.
\end{lem}

\begin{proof}
    For each $0 \le i \le \nbSubClasses$, we have $\objFun{i}{\TestSuite_1} \le \objFun{i}{\TestSuite_2}$ and $\objFun{i}{\TestSuite_2} \le \objFun{i}{\TestSuite_3}$, so $\objFun{i}{\TestSuite_1} \le \objFun{i}{\TestSuite_3}$.
    Moreover, there exists $0 \le i_1 \le \nbSubClasses$ such that $\objFun{i_1}{\TestSuite_1} < \objFun{i_1}{\TestSuite_2} \le \objFun{i_1}{\TestSuite_3}$ and there exists $0 \le i_2 \le \nbSubClasses$ such that $\objFun{i_2}{\TestSuite_1} \le \objFun{i_2}{\TestSuite_2} < \objFun{i_2}{\TestSuite_3}$.
    $i_1$ and $i_2$ can be the same or distinct.
    In any case, we have $\objFun{i_1}{\TestSuite_1} < \objFun{i_1}{\TestSuite_3}$ and $\objFun{i_2}{\TestSuite_1} < \objFun{i_2}{\TestSuite_3}$.
\end{proof}

\begin{lem}
\label{theo:miserDom}
    For every generation $n$, if $\TestSuite_0 \in \Misers{n} \setminus \Misers{n + 1}$, then there exists $\TestSuite \in \Misers{n + 1}$ such that $\TestSuite \dominates \TestSuite_0$, where $\dominates$ is the domination relation from (\S II-E). % \Cref{defi:pareto}.
\end{lem}

\begin{proof}
In the miser population update (\S VIII-F), % (\Cref{sec:aim:updtPops}),
$\TestSuite_0$ can be removed from the miser population only if there exists a miser candidate $\TestSuite_1$ such that $\TestSuite_1 \dominates \TestSuite_0$.
If $\TestSuite_1$ is accepted in the population then $\TestSuite = \TestSuite_1$ satisfies the \namecref{theo:miserDom}.

Otherwise, $\TestSuite_1$ is rejected only because there exists a miser $\TestSuite_2$ such that $\TestSuite_2 \dominates \TestSuite_1$.
Hence, according to \Cref{theo:ParetoDomTransitive}, we have by transitivity that $\TestSuite_2 \dominates \TestSuite_0$.
Note that there is at most two miser candidates per generation.
If either $\TestSuite_1$ is the only miser candidate or there exists a second miser candidate $\TestSuite_3$ which does not dominate $\TestSuite_2$, then $\TestSuite_2$ is present in the next generation and $\TestSuite = \TestSuite_2$ satisfies the \namecref{theo:miserDom}.

Otherwise, there exists a second candidate $\TestSuite_3$ such that $\TestSuite_3 \dominates \TestSuite_2$.
Hence, according to \Cref{theo:ParetoDomTransitive}, we have by transitivity that $\TestSuite_3 \dominates \TestSuite_0$.
If $\TestSuite_3$ is accepted in the population then $\TestSuite = \TestSuite_3$ satisfies the \namecref{theo:miserDom}.

Otherwise, $\TestSuite_3$ is rejected only because there exists a miser $\TestSuite_4$ such that $\TestSuite_4 \dominates \TestSuite_3$.
Hence, according to \Cref{theo:ParetoDomTransitive}, we have by transitivity that $\TestSuite_4 \dominates \TestSuite_0$.
Because there is at most two miser candidates per generation, $\TestSuite_4$ cannot be removed by another candidate.
Therefore, $\TestSuite_4$ is present in the next generation and $\TestSuite = \TestSuite_4$ satisfies the \namecref{theo:miserDom}.
\end{proof}

\begin{cor}[Dominance across Generations]
\label{theo:miserTemporalDom}
    For every generation $n$ and for every $\TestSuite_1 \in \Misers{n}$, if there exists $0 \le m \le n$ and $\TestSuite_2 \in \Misers{m}$ such that $\TestSuite_2 \dominates \TestSuite_1$, then there exists $\TestSuite_3 \in \Misers{n}$ such that $\TestSuite_3 \dominates \TestSuite_1$.
\end{cor}

\begin{proof}
The proof is done by induction on $n - m$.

If $\TestSuite_2 \in \Misers{n}$ then $\TestSuite_2 = \TestSuite_3$ satisfies the \namecref{theo:miserTemporalDom}.

Otherwise, there exists a generation $m < g \le n$ where $\TestSuite_2$ was removed.
In that case, according to \Cref{theo:miserDom}, there exists $\TestSuite_3 \in \Misers{g}$ such that $\TestSuite_3 \dominates \TestSuite_2$.
Hence, according to \Cref{theo:ParetoDomTransitive}, we have by transitivity that $\TestSuite_3 \dominates \TestSuite_1$.
Finally, because $n - g < n - m$, we have the result using the induction hypothesis on $\TestSuite_3$.
\end{proof}

We finally prove, as expected, the properties satisfied by misers on each generation.

\begin{theo}[Invariant of the Misers]
\label{theo:misers}
\label{theo:appendix:misers}
    For every generation $n$, for every $\TestSuite_1 \in \Misers{n}$, we have:
    \begin{itemize}
        \item $\TestSuite_1$ is reduced (in the sense of \S III-C) % \Cref{defi:reduction})
        \item $\getSubclasses{\TestSuite} \subset \Objectives(\RedComp)$ (the inclusion is strict)
        \item There exists no $\TestSuite_2 \in \bigcup\limits_{0 \le m \le n} \Misers{m}$ such that $\TestSuite_2 \dominates \TestSuite_1$.
    \end{itemize}
\end{theo}

\begin{proof}
The initial miser population is empty (\S VIII-B), % (\Cref{sec:aim:initPops}),
hence the properties trivially hold.

After mutation (\S VIII-E) % (\Cref{sec:aim:mutation})
each offspring $\TestSuite$ is replaced by its reduced counterpart $\reduction{\TestSuite}$ before determining if it is accepted in the miser population or rejected.
Hence, for each generation, each miser is reduced.

In the miser population update (\S VIII-F), % (\Cref{sec:aim:updtPops}),
an offspring can be a candidate to the miser population only if it does not cover all the objectives.

Finally, the last property is proved for a miser $\TestSuite_1 \in \Misers{n}$.
Let $n'$ be the first generation when $\TestSuite_1$ was accepted, so we have $n' \le n$ and $\TestSuite_1 \in \Misers{n'}$.

The proof is done by contradiction, assuming that there existed a generation $0 \le m \le n$ and a miser $\TestSuite_2 \in \Misers{m}$ such that $\TestSuite_2 \dominates \TestSuite_1$.
Let $m'$ be the first generation when $\TestSuite_2$ was accepted, so we have $m' \le m$ and $\TestSuite_2 \in \Misers{m'}$.
We consider two cases.

If $m' \le n'$ then, according to \Cref{theo:miserTemporalDom}, there exists $\TestSuite_3 \in \Misers{n'}$ such that $\TestSuite_3 \dominates \TestSuite_1$.
This contradicts the above procedure, because if $\TestSuite_1$ was dominated it would not have been accepted in $\Misers{n'}$.

If $m' > n'$ then, because $\TestSuite_2 \dominates \TestSuite_1$, according to the above procedure $\TestSuite_1$ is removed so $\TestSuite_1 \not\in \Misers{m'}$.
But $m' \le m \le n$ and $\TestSuite_1 \in \Misers{n}$, so $\TestSuite_1$ was added between $m'$ and $n$.
Let $g$ be the first generation when this occurred.

In that case we have $\TestSuite_1 \in \Misers{g}$, $0 \le m' \le g$, $\TestSuite_2 \in \Misers{m'}$, and $\TestSuite_2 \dominates \TestSuite_1$.
So, according to \Cref{theo:miserTemporalDom}, there exists $\TestSuite_3 \in \Misers{g}$ such that $\TestSuite_3 \dominates \TestSuite_1$, which contradicts the fact that $\TestSuite_1$ was accepted in $\Misers{g}$.
\end{proof}


==> Figures/redundantComponentsA.tex <==
\begin{tikzpicture}[scale=1.5]
    % styles
    \tikzset{
        component/.style={very thick},
		edge/.style={thick,color=black},
    }
    % sequences
    \node[red]
        (seq1)
        at (-1,1)
        {$\sequence_1$};
    \node[red]
        (seq2)
        at (-1,0)
        {$\sequence_2$};
    \node[red]
        (seq3)
        at (-1,-1)
        {$\sequence_3$};
    \node[blue]
        (seq4)
        at (0,-1)
        {$\sequence_4$};
    \node[red]
        (seq5)
        at (1,-1)
        {$\sequence_5$};
    \node[red]
        (seq6)
        at (1,0)
        {$\sequence_6$};
    % sequences
	\draw[edge]
        (seq1) -- (seq2);
	\draw[edge]
        (seq2) -- (seq3);
	\draw[edge]
        (seq3) -- (seq4);
	\draw[edge]
        (seq4) -- (seq5);
	\draw[edge]
        (seq5) -- (seq6);
\end{tikzpicture}


==> Figures/redundantComponentsB.tex <==
\begin{tikzpicture}[scale=1.5]
    % styles
    \tikzset{
        component/.style={very thick},
		edge/.style={thick,color=black},
    }
    % sequences
    \node[red]
        (seq1)
        at (-1,1)
        {$\sequence_1$};
    \node[red]
        (seq2)
        at (-1,0)
        {$\sequence_2$};
    \node[red]
        (seq3)
        at (-1,-1)
        {$\sequence_3$};
    \node[red]
        (seq5)
        at (1,-1)
        {$\sequence_5$};
    \node[red]
        (seq6)
        at (1,0)
        {$\sequence_6$};
    % components
    \draw[component,red]
        (seq1.north west) --
        (seq1.north east) --
        (seq3.south east) --
        (seq3.south west) --
        cycle;
    \draw[component,red]
        (seq6.north west) --
        (seq6.north east) --
        (seq5.south east) --
        (seq5.south west) --
        cycle;
    % sequences
	\draw[edge]
        (seq1) -- (seq2);
	\draw[edge]
        (seq2) -- (seq3);
	\draw[edge]
        (seq5) -- (seq6);
\end{tikzpicture}


==> Preamble/theoremStyles.tex <==
\theoremstyle{plain}
\newtheorem{theo}{Theorem}%[section]
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{claim}{Claim}

\theoremstyle{definition}
\newtheorem{defi}{Definition}
\newtheorem{ex}{Example}

\theoremstyle{remark}
\newtheorem*{rem}{Remark}



==> tables/ActionClusteringResults.tex <==
% \begin{table*}[tb]

% \centering
% \caption{Action clustering results}
% \resizebox{\textwidth}{!}{%
% \label{tab:actionClusteringResults}
% \small
% \begin{tabular}{|cc|ccc|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Output Clustering}}} &
%   \multicolumn{3}{c|}{\textbf{Action Clustering}} \\ \cline{3-5} 
% \multicolumn{2}{|c|}{} &
%   \multicolumn{1}{c|}{\textbf{Kmeans}} &
%   \multicolumn{1}{c|}{\textbf{Dbscan}} &
%   \textbf{Hdbscan} \\ \hline
% \multicolumn{1}{|c|}{\textbf{Clustering algorithms}} &
%   \textbf{Distance functions} &
%   \multicolumn{1}{c|}{\textbf{Number of action subClasses}} &
%   \multicolumn{1}{c|}{\textbf{Number of action subClasses}} &
%   \textbf{Number of action subClasses} \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Kmeans}}} &
%   \textbf{Levenshtein} &
%   \multicolumn{1}{c|}{62} &
%   \multicolumn{1}{c|}{56} &
%   97 \\ \cline{2-5} 
% \multicolumn{1}{|c|}{} &
%   \textbf{Bag} &
%   \multicolumn{1}{c|}{59} &
%   \multicolumn{1}{c|}{54} &
%   91 \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Dbscan}}} &
%   \textbf{Levenshtein} &
%   \multicolumn{1}{c|}{69} &
%   \multicolumn{1}{c|}{60} &
%   83 \\ \cline{2-5} 
% \multicolumn{1}{|c|}{} &
%   \textbf{Bag} &
%   \multicolumn{1}{c|}{62} &
%   \multicolumn{1}{c|}{56} &
%   81 \\ \hline
% \end{tabular}%
% }
% \end{table*}


\begin{table}[t]
\centering
\caption{Number of action subclasses for each clustering algorithm for \jenkins}
\label{tab:actionClusteringResults}

\begin{tabular}{|cc|ccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Output Clustering}} & \multicolumn{3}{c|}{Action Clustering}                              \\ \cline{3-5} 
\multicolumn{2}{|c|}{}                                   & \multicolumn{1}{c|}{Kmeans} & \multicolumn{1}{c|}{DBSCAN} & HDBSCAN \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{K-means}} & Levenshtein& \multicolumn{1}{c|}{62} & \multicolumn{1}{c|}{56} & 97 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}               & Bag               & \multicolumn{1}{c|}{59}     & \multicolumn{1}{c|}{54}     & 91      \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{DBSCAN}}  & Levenshtein & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{60} & 83 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}               & Bag               & \multicolumn{1}{c|}{62}     & \multicolumn{1}{c|}{56}     & 81      \\ \hline
\end{tabular}%

\end{table}


==> tables/ExecutionTime.tex <==
\begin{table}[t]
\centering
\caption{Execution time of the MRs with the initial input set and the minimized input set on Jenkins}
\label{tab:ExecutionTime}
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |}
\hline
\cellcolor[HTML]{FFFFFF}                     & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}Execution time (minutes)}        \\ \cline{2-3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}MR ID} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}initial input set} & minimized input set\\ \hline
CWE\_863           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}520}  & 327 \\
CWE\_22           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}33}    & 8   \\
CWE\_280           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}472} & 11  \\
CWE\_284           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}54}   & 15  \\
CWE\_286           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}236}  & 15 \\
CWE\_420           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}63}   & 16 \\
CWE\_434           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3}    &   1  \\
CWE\_923           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}    & 1   \\
OTG\_AUTHZ\_003    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}22}   & 1  \\
OTG\_BUSLOGIC\_005 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6}    & 1   \\
CWE\_200           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}    & 1   \\ \hline
Total              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}913}   & 370  \\ \hline
\end{tabular}%
\end{table}

==> tables/ExecutionTimeJoomla.tex <==
\begin{table}[t]
\centering
\caption{Execution time of the MRs with the initial input set and the minimized input set on Joomla}
\label{tab:JoomlaExecutionTime}
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |}
\hline
\cellcolor[HTML]{FFFFFF}                     & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}Execution time (minutes)}        \\ \cline{2-3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}MR ID} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}initial input set} & minimized input set\\ \hline
CWE\_266           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}520}  & 318 \\
CWE\_276           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}7}    & 1   \\
CWE\_280           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ongoing} & ongoing  \\
CWE\_284           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}54}   & 15  \\
CWE\_286           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}236}  & 15 \\
CWE\_420           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}63}   & 16 \\
CWE\_434           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3}    &   1  \\
CWE\_923           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}    & 1   \\
OTG\_AUTHZ\_003    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}22}   & 1  \\
OTG\_BUSLOGIC\_005 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}6}    & 1   \\
CWE\_200           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}    & 1   \\ \hline
Total              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}913}   & 370  \\ \hline
\end{tabular}%
\end{table}

==> tables/OutputClusteringResult.tex <==
\begin{table}[tb]
\small % Reduce the font size
\centering
\caption{Jenkins output clustering results}
\label{tab:OutputClaustering}
\begin{tabular}{c c|c|c|c|c|}
\cline{3-6}
 & &
  \multicolumn{4}{c|}{Distance}\\
\cline{3-6}
 & &
  \multicolumn{2}{c|}{Levenshtein} &
  \multicolumn{2}{c|}{Bag} \\
\cline{3-6} 
 & &
  \multicolumn{1}{c|}{Hyper-} &
  \text{Number} &
  \multicolumn{1}{c|}{Hyper-} &
  \text{Number} \\ 
& &
  \multicolumn{1}{c|}{parameter(s)} &
  \text{of clusters} &
  \multicolumn{1}{c|}{parameter(s)} &
  \text{of clusters} \\
\hline
\multicolumn{1}{|c|}{} & \kmeans & \multicolumn{1}{c|}{$K = 42$}            & 42               & \multicolumn{1}{c|}{$K = 40$}           & 40               \\ \cline{2-6}
\multicolumn{1}{|c|}{Algorithm} & \dbscan & \multicolumn{1}{c|}{$\minpts = 1$, $\epsilon = 4.92$} & 53               & \multicolumn{1}{c|}{$\minpts = 1$, $\epsilon = 4.5$} & 50               \\
\cline{2-6}
\multicolumn{1}{|c|}{} & \hdbscan & \multicolumn{1}{c|}{$n = 2$}             & 98 & \multicolumn{1}{c|}{$n = 2$}            & 102 \\
\hline
\end{tabular}
\end{table}


==> tables/joomla_ActionClustering.tex <==
\begin{table}[tb]
\centering
\caption{Number of action subclasses for each clustering algorithm for \joomla}
\label{tab:joomlaActionClusteringResults}

\begin{tabular}{|cc|ccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Output Clustering}} & \multicolumn{3}{c|}{Action Clustering}                              \\ \cline{3-5} 
\multicolumn{2}{|c|}{}                                   & \multicolumn{1}{c|}{Kmeans} & \multicolumn{1}{c|}{DBSCAN} & HDBSCAN \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{K-means}} & Levenshtein& \multicolumn{1}{c|}{102} & \multicolumn{1}{c|}{58} & 95 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}               & Bag               & \multicolumn{1}{c|}{95}     & \multicolumn{1}{c|}{57}     & 92      \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{DBSCAN}}  & Levenshtein & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{62} & 67 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}               & Bag               & \multicolumn{1}{c|}{73}     & \multicolumn{1}{c|}{50}     & 84      \\ \hline
\end{tabular}%

\end{table}


==> tables/joomla_OutputClustering.tex <==
\begin{table}[tb]
\small % Reduce the font size
\centering
\caption{Joomla output clustering results}
\label{tab:JoomlaOutputClaustering}
\begin{tabular}{c c|c|c|c|c|}
\cline{3-6}
 & &
  \multicolumn{4}{c|}{Distance}\\
\cline{3-6}
 & &
  \multicolumn{2}{c|}{Levenshtein} &
  \multicolumn{2}{c|}{Bag} \\
\cline{3-6} 
 & &
  \multicolumn{1}{c|}{Hyper-} &
  \text{Number} &
  \multicolumn{1}{c|}{Hyper-} &
  \text{Number} \\ 
& &
  \multicolumn{1}{c|}{parameter(s)} &
  \text{of clusters} &
  \multicolumn{1}{c|}{parameter(s)} &
  \text{of clusters} \\
\hline
\multicolumn{1}{|c|}{} & \kmeans & \multicolumn{1}{c|}{$K = 45$}            & 45               & \multicolumn{1}{c|}{$K = 44$}           & 44               \\ \cline{2-6}
\multicolumn{1}{|c|}{Algorithm} & \dbscan & \multicolumn{1}{c|}{$\minpts = 1$, $\epsilon = 14.83$} & 43               & \multicolumn{1}{c|}{$\minpts = 1$, $\epsilon = 13.17$} & 42               \\
\cline{2-6}
\multicolumn{1}{|c|}{} & \hdbscan & \multicolumn{1}{c|}{$n = 2$}             & 61 & \multicolumn{1}{c|}{$n = 2$}            & 62 \\
\hline
\end{tabular}
\end{table}


==> tables/tableHyperParamOutputClustering.tex <==
\begin{table}[t]
\centering
\caption{Value of hyper-parameters of the clustering algorithms for output clustering \textbf{\textcolor{Orange}{YM: Tables should not overlap the margin, please do not use resizebox}}}
\label{tab:HyperParamOutputClaustering}
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{|c|cc|}
\hline
\multirow{1}{*}{\textbf{Clustering algorithm}} 
 &
  \multicolumn{1}{c|}{\textbf{$\lev$ distance }} &
 
  \multicolumn{1}{c|}{\textbf{Bag Distance}}  \\ \hline
\textbf{K-means} & \multicolumn{1}{c|}{K = 42}                         & \multicolumn{1}{c|}{K = 40}                        \\ \hline
\textbf{Dbscan}  & \multicolumn{1}{c|}{n = 1, $\epsilon$ = 4.92}                & \multicolumn{1}{c|}{n = 1, $\epsilon$ = 4.5}                \\ \hline
\textbf{Hdbscan} & \multicolumn{1}{c|}{n = 2}              & \multicolumn{1}{c|}{n = 2}            \\ \hline
\end{tabular}%
}
\end{table}

==> tables/tableVulnerabilities.tex <==

%\begin{table}[htb]
\begin{table}[t]
\center
\scriptsize
\caption{Vulnerabilities considered in our empirical evaluation. \textbf{\textcolor{Orange}{YM: I don't see the point of the Jenkins column since there is only one value, hence you can just indicate in the caption that this is about Jenkins. Moreover there's one ref per vulnerability, so you can use a cite command just after the id. You should add to each id a hyperlink leading to the CVE description in the CVE website. The separation between the descriptions is not clear, so please ad hline or cline commands between them.}}}
\label{table:subjectVulnrabilities}
\begin{tabular}{|r|r|p{2cm}|p{4cm}|}
\hline
%\multicolumn{1}{|c|}{\textbf{Security Design}} &

 % \textbf{\begin{tabular}[c]{@{}l@{}}\% of addressed \\ weaknesses\end{tabular}}  
  \textbf{Subject} &
  \textbf{Ref.} & \textbf{CVE Id} &
    \textbf{Description} 
 \\ 
 \hline
\multirow{9}{*}{Jenkins} &
  \ cite{JV6} %9003
  &
 % \NB{why we have this?CWE\_863},
  % CWE\_280 &
   CVE-2018-1999003 &
  Jenkins does not perform a permission check for URLs handling cancellation of queued builds, allowing users with Overall/Read permission to cancel queued builds. \\
 &
 % CVE-2018-1999004 
 \ cite{JV5}&
 % CWE\_863, CWE\_285 , \NB{also see 286} 
 CVE-2018-1999004 &

  Jenkins does not perform a permission check for the URL that initiates agent launches,
  allowing users with Overall/Read permission to initiate agent launches. \\
 &

 % CVE-2018-1000406 
 \ cite{JV9}&
  % CWE\_276 (\NB{it was 22}) 
CVE-2018-1000406  &
  In the file name parameter of a Job configuration, users with Job/Configure permissions can specify a relative path escaping the base directory. Such path can be used to upload a file on the Jenkins host, resulting in an arbitrary file write vulnerability. \\
 &
 % CVE-2018-1999046 
 \ cite{JV2}&
  % CWE\_286 (\NB{it was 200}) 
  CVE-2018-1999046 &
  Users with Overall/Read permission are able to access the URL serving agent logs on the UI due to a lack of permission checks. \\


  
\hline
\end{tabular}
\end{table}


==> tables/test.tex <==
\begin{table}[th]
\centering
\footnotesize
\caption{Comparison of genetic algorithms for \jenkins.}
\label{tab:jenkins:algos}
\begin{tabular}{cc|c|c|c|}
\hline
\multicolumn{2}{|c|}{costs} & \geneticAlgo & \mosa & \nsgaThree \\
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\geneticAlgo}} & $\pValue$
	 & 
	 & \cellcolor{green!100}\num{8.9e-16}
	 & \cellcolor{green!100}\num{8.9e-16}\\
\multicolumn{1}{|c|}{} & $\effectSize$
	 & 
	 & \cellcolor{green!100}0.0
	 & \cellcolor{green!100}0.0\\
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\mosa}} & $\pValue$
	 & \cellcolor{red!100}\num{8.9e-16}
	 & 
	 & \num{1.0e+00}\\
\multicolumn{1}{|c|}{} & $\effectSize$
	 & \cellcolor{red!100}1.0
	 & 
	 & 0.72\\
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\nsgaThree}} & $\pValue$
	 & \cellcolor{red!100}\num{8.9e-16}
	 & \num{1.0e+00}
	 & \\
\multicolumn{1}{|c|}{} & $\effectSize$
	 & \cellcolor{red!100}1.0
	 & 0.28
	 & \\
\hline
\end{tabular}
\end{table}

